Assessing Intel's Memory Bandwidth Allocation for resource limitation in real-time systems

Industries are recently considering the adoption of cloud computing for hosting safety critical applications. However, the use of multicore processors usually adopted in the cloud introduces temporal anomalies due to contention for shared resources, such as the memory subsystem. In this paper we explore the potential of Intel's Memory Bandwidth Allocation (MBA) technology, available on Xeon Scalable processors. By adopting a systematic measurement approach on real hardware, we assess the indirect memory bandwidth limitation achievable by applying MBA delays, showing that only given delay values (namely 70, 80 and 90) are effective in our setting. We also test the derived bandwidth assured to a hypothetical critical core when interfering cores (e.g., generating a concurrent memory access workload) are present on the same machine. Our results can support designers by providing understanding of impact of the shared memory to enable predictable progress of safety critical applications in cloud environments.

==> Intel-MBA-Assessment ISORC_2022/conclusion.tex <==
MBA is an interesting and reliable hardware feature for resource limitation in real-time systems. It can be used to regulate the access contention by limiting the arrival rate of the single physical cores. %Such regulation is more straightforward to evaluate than other hardware approaches that introduce a quality of service in the network of interconnect.} \newline
In this paper, we provide a systematic approach to estimate the indirect limitation of the MBA using three main workloads: memory reads with no L2 writebacks, memory reads with L2 writebacks and memory reads with L2 writebacks and memory writes.
With experiments conducted on real hardware we discover that a good approach to measure the limitation in the worst-case is to run measurements without L2 writebacks. In addition, we found that  only the Intel's 70, 80, and 90 delays values lead to significant limitations un our setting. Such limitation for the maximum synchronous bandwidth continues to be valid when there are memory writes, differently from state-of-the-art software-based solutions such as Memguard \cite{Yun2013MemGuardMB}. \newline
Our evaluation in the multi-core analysis showed that the MBA is able to provide memory bandwidth isolation for a critical task under heavy memory-intensive workloads on multi-core platforms. In addition, the MBA enables short regulation periods that would be hardly achievable with software-based methods.  Finally, the MBA hardware limitation does not require to stop the execution of interfering cores to prevent memory accesses, and it does not require to execute the periodic regulation subroutine, improving the overall efficiency. Although results are achieved for a specific processor, we believe the proposed method is general enough to be applicable on different processor models.\newline
In the future, we plan to design a MBA-based approach to regulate the memory demand based on the current status of the memory controller and requirements of critical tasks, by dynamically assigning the required delay to interference cores, approaching an efficient regulation algorithm.

==> Intel-MBA-Assessment ISORC_2022/design_of_exp.tex <==
%\textbf{\todo[inline]{Temporary UNLOCK: TUKL}}
%\todo[inline]{GF: we should provide data on the statistical quality of the data, eg, confidence intervals (DONE We put the boxplots avoiding the huge table)}
%\todo[inline]{GG: at some point we should mention exactly which processor (name) we used}
We design a set of experiments to perform two main analyses.
The single-core analysis is based on a systematic approach to deriving the indirect memory bandwidth limitation achieved when the MBA delays the requests. 
Contrarily, the multi-core analysis is focused on the guarantees rather than the limitation.
Multi-core analysis tests the memory bandwidth achieved by a core executing a critical VM when the MBA (indirectly) limits memory accesses from 3 interfering cores (performing best-effort tasks).
Both, single-core and multi-core analysis, share the following architectural parameters (Table \ref{tab:share_parameters}). We use only one socket (one processor) composed of eight cores at most. We set the number of active cores via BIOS configuration. We only used one memory channel in both analyses. 
%One DRAM channel throughput seems to satisfy the core arrival rate. 
%In this architecture, six channels are pluggable at most. 
We set the DRAM refresh rate to periodic and the CPU core frequency to maximum (no power saving) in the BIOS. These parameters helped keep the latency variability to a minimum and maximize the memory requests rate. Similarly, we disabled the Pre-fetcher and Hyperthreading to reduce variability since hardware threads on the same physical core share the same “queue” to the memory, while the prefetcher can preload several lines after a single cache miss. 
Experiments are conducted on an Intel Xeon Silver processor, Cascade-Lake microarchitecture, with 8 cores, 2,10 GHz, 512KB L1 cache (256KB out of 512 KB are dedicated for the Code), 1MB L2 cache, and 11MB LLC. %\todo[inline]{For Gautam: exactly which is the model of the processor?(we didn't remember the exactly model of processor, we should execute "cat /proc/cpuinfo" on the processor (it is a CPUID command) to see the model)}
Next subsections present the design of experiments for both analyses. Our measures achieve \sout{the} 99\% of accuracy calculated as the 99\% mean confidence interval using a student's t distribution divided by the sample mean.
\begin{table}
\caption{Design of experiments: shared parameters \label{tab:share_parameters}}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
\textbf{Shared parameters} & \textbf{setting}
\tabularnewline
\hline 
\hline 
Sockets no. & 1
\tabularnewline
\hline 
Used DRAM channel & 1
\tabularnewline
\hline 
Prefetcher & disabled 
\tabularnewline
\hline 
SMT &disabled
\tabularnewline
\hline
DRAM refresh cycles & periodic
\tabularnewline
\hline
Core frequency &Maximum
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


\subsection{Single-core analysis}
Single-core analysis has the objective to estimate the memory access limit for an interfering core when MBA is enabled with different delays. We exclude 20 and 30 delays from the analysis as they are erroneous on our processor (as reported in an Intel errata \cite{IntelRefManXeonScal}) and produce the same results as delay value 10.
Table \ref{tab:doe_onecoreanalysis} describes the design of experiments of the single-core analysis. Our experiments measure the latency execution variability for different kinds of workloads: memory read workload considers only synchronous memory accesses, while memory write workload accounts also the asynchronous memory writes. One of the main contributions is to specialize the memory read workload regarding the L2 writebacks as motivated later.  The number of observations achieves more than 99\% of accuracy.

\begin{table}
\caption{Design of experiments: single-core analysis \label{tab:doe_onecoreanalysis}}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
%\textbf{Goal} & Quantify and evaluate the MBA \\ &throttling without memory interference
%\tabularnewline
%\hline 
%\hline 
\textbf{Parameters} & \textbf{setting}
\tabularnewline
\hline 
Cores no. & 1 
\tabularnewline
\hline 
\hline 
\textbf{Factors} & \textbf{values}
\tabularnewline
\hline 
MBA delay& $d\in D, D=\{10; 40; 50; 60; 70; 80; 90\}$
\tabularnewline
\hline
Workload &$k \in K, K=\{R^{I}; R^{II}; W^{II}\}$\\& \begin{tabular}{ c c c }
$R^{I}:$ \{&$R^{II}$: \{ &$W^{II}$: \{ \\8192  CAS R,&8192 CAS  R,&8192  CAS R,
\\no  L2WBs,&with  L2WBs,&with  L2WBs,
\\no LLCWBs\}&no LLCWBs\}&with LLCWBs \}
\end{tabular}
\tabularnewline
\hline 
\hline 
\textbf{Metric} & \textbf{description}
\tabularnewline
\hline 
Memory & memory fetching latency in terms of CPU cycles\\fetching&
$L_{k;d}$, $k \in K, d \in D$ \\latency &
%\tabularnewline
%\hline
%\textbf{Obs. no.} & $30$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


\subsubsection{Memory read workload}
A read request in the worst case corresponds to a memory read operation when there is an LLC miss. Since we consider this worst-case in our workload, read request and memory read operation are interchangeable terms.\newline
However, we identify two different L2 traffic patterns for this worst-case due to the LLC exclusivity in the processor. \newline
In the exclusive architecture, L2 writebacks (L2WBs) to the LLC happen whenever new memory is read and the L2 set is full, even though the evicted L2 cache line is clean (contrarily to the inclusive architecture). 

\begin{figure}[t!]
\centering
\includegraphics[width=.48\textwidth]{pictures/fineg_mba_thrott_latency_continuous_64KB_memory_fetching_delay0} \
\caption{2048 KB memory fetching in several blocks of 64KB when the MBA is disabled (0-delay)\label{fig:fineg_l2_wb_00}}
\end{figure}
\begin{figure}[t!]
\centering
\includegraphics[width=.48\textwidth]{pictures/fineg_mba_thrott_latency_continuous_64KB_memory_fetching_delay9} \
\caption{2048 KB memory fetching in several blocks of 64KB when the MBA 90-delay is enabled\label{fig:fineg_l2_wb_90}}
\end{figure}

%The new Xeon processors (our micro-architecture) have an exclusive LLC.
We include the two L2 traffic patterns as a factor motivating this choice in Fig.\ref{fig:fineg_l2_wb_00} and Fig.\ref{fig:fineg_l2_wb_90} where we fetch 2 MB of dynamic memory in several blocks of 64 KB when the MBA is disabled (0-delay) and enabled with 90-delay. 
While the above plot represents the latency (CPU cycles) for each block, the graph below shows the respective L2WBs for each fetched block. The number of L2WBs grows as the L2 cache fills its capacity (L2 size is 1 MB). While initially, no L2WBs are observed (when L2 capacity is available), subsequently, when the L2 becomes full, each memory read will sure correspond to one L2WB (so 1024 memory reads of 64 bytes (64KB) generate 1024 L2 writebacks). \newline
Looking at the figures, we have two main observations. (i) Without throttling (0-delay), the memory load latency does not change significantly when the L2WBs are present (Fig.\ref{fig:fineg_l2_wb_00})\footnote{Note that our memory read workloads are designed to not cause LLC writebacks (LLCWBs)}. However, (ii) the latency changes when the MBA is enabled (Fig.\ref{fig:fineg_l2_wb_90}) on the two traffic patterns. From the results on CPU cycles, it is evident that the MBA delays the L2WBs requests, doubling the latency of read operations when writebacks are present. 
%This explanation is plausible 
This might be possible because the controller should introduce a delay towards all outgoing requests on the interconnection network, thus also including reads and writes to the last level cache. \newline
The second observation motivates us to consider L2 traffic pattern as a factor. The $R^{I}$ and $R^{II}$ in Table \ref{tab:doe_onecoreanalysis} represent the read workload respectively in the first (without L2WBs) and the second operational condition (with L2WBs). 
In particular, the read workload is composed of 8192 read requests where each request is an LLC miss ($ readReqs = LLC misses = CAS Reads = 8192$) and hence a memory read operation (CAS R is the command issued on the DRAM channel). The number of 8192 requests (meaning 512KB of memory fetching  because each request retrieves 64 bytes which is the cache line size) has been chosen since it assures us to not have L2WBs in $R^{I}$ ($L2WBs = 0$), given the L2 cache size of 1MB. This is also visible from Fig.\ref{fig:fineg_l2_wb_00}, where after 8 fetchings of 64 KB each, the number of L2WBs is still 0.
On the opposite, in $R^{II}$ the total L2 write-backs must be equal to the total memory requests ($L2 WBs=8192$). This is achieved by performing a pre-read workload to fill the L2 cache.
%These equalities serve as a validation test.
Note that, considering the results in Fig.\ref{fig:fineg_l2_wb_00} and Fig.\ref{fig:fineg_l2_wb_90}, $R^{I}$ is the worst case workload (it has less limitation), since the frequency (latency) of memory reads is not reduced (delayed) by concurrent L2WBs. %We use this observation to set $R^{I}$ as the worst-case interfering workload for the multicore analysis.

As a side note, looking at Fig.\ref{fig:fineg_l2_wb_90}, we can observe that the MBA keeps the same limitation for each of the 1024 memory reads. Such workload in software-based approaches would require to set an infeasible regulation period of 10 microseconds, hence proving the better granularity offered by MBA-based approaches.

\subsubsection{Memory write workload}

We have memory writes in a writeback policy when a dirty LLC cache line is evicted.
%write requests on miss cache lines in a writeback policy are memory reads operations until a dirty LLC cache line is evicted, causing a memory write. 
Hence, since our write workload reproduces the worst case, every request of the workload causes one memory read and one memory write operation, due to the cache line eviction and substitution. %The worst case of write requests has only one possible L2 operational condition (i.e., only the second with L2WBs)  because an LLC writeback is the effect of an L2 writeback.
The $W^{II}$ in  Table \ref{tab:doe_onecoreanalysis} represents this kind of workload.
In particular, the $W^{II}$ workload is composed of 8192 requests where each request is the cause of one memory read, and one memory write ($ writeReqs = LLCmisses = CAS Reads = CAS Writes = 8192$). Only the second operational condition ($II$) is possible for the write workload since an LLC writeback can only be the result of a L2 writeback.
%Again, these equalities serve as a validation test.
%In conclusion the one-core analysis consists to evaluate the memory fetching latency when the MBA delays and traffic patterns change.

\subsection{Multi-core analysis}
While the single-core analysis gives us information about the memory access limitation when the MBA delay and workload are fixed, the multi-core analysis analyzes the assured memory fetching latency for a critical core when the MBA limits the accesses of the other cores. 
For our evaluation, we deploy a quad-core system where one of them is critical.\newline
In particular, we consider a specific case where the critical core fetches its dynamic memory without MBA limitation, reproducing a workload $R^{I}$. In contrast, the MBA limits the other three cores that perform the most permissive workload $k'$ under limitation resulting by the single-core analysis.
%in their interference workloads (also set to $R^{I}$, but with a larger fetching set to 728KB = 12288 reads, to produce a worst-case interference lasting longer than the critical workload). \newline
The range of delays considered for the interference cores range from 10 to 90, however we will consider only significant ones $D'$, depending on the result of single-core analysis. The Table \ref{tab:doe_multicoreanalysis} describes the design of experiments. The multi-core analysis requires thirty observations to achieve a 99\% of accuracy.
%In addition, we explain the observed data through an interpretive model.
\subsection{Measurement tool and workload considerations \label{measuremnt_tool}}
We performed experiments in Linux as the high server boot duration (several minutes) makes it time-consuming to do bare-metal development and experimentation. \newline
Our measurement tool captures the latency and several factors (such as LLC writeback, L2 writeback, and CAS commands) of a particular workload. The latency is captured in terms of TSC (Timestamp counter). The fixed TSC frequency is close to the maximum CPU frequency. Hence, we refer to TSC cycles as CPU cycles. We favor the latency rather than bandwidth measurements because the latter requires a regulation period limiting the resolution. \newline
We maximize the interference writing the workload as consecutive memory operations (full-loop unrolling) and choosing a stride between consecutive accesses equal to the cache line size (our cache line size is 64 Bytes). Even though the loop unrolling of memory requests increases the code size, we design our experiments controlling the absence of extra LLC misses. \newline
We reproduce the L2 traffic patterns for a read workload through initial setup operations. To avoid L2 writebacks and to have memory accesses, we flush the dynamic memory before the workload execution, while to reproduce L2 writebacks for the $R^{II}$ workload, we also perform a pre-read workload to fill the L2 cache, as previously mentioned. \newline
Contrarily, for the write workload $W^{II}$, we reproduce the worst-case executing a pre-workload of write-requests filling the entire cache space of dirty and useless cache-lines. In addition to synchronous memory accesses, the previous injected dirty cache lines assure LLC writeback (memory write) whenever an LLC eviction occurs.



\begin{table}
\caption{Design of experiments: multi core analysis \label{tab:doe_multicoreanalysis}}
\begin{center}
\begin{tabular}{ |c| c| }
%\hline 
%\textbf{Goal} & Quantify and explain \\& the critical core assured bandwidth \\& when the MBA limits the interference\\& cores with significant delays
%\tabularnewline
%\hline 
\hline 
\textbf{Parameters} & \textbf{setting}
\tabularnewline
\hline 
crit. cores no. & $1$
\tabularnewline
\hline
crit. workload & $R^{I}$
\tabularnewline
\hline 
int. cores no. & $3$
\tabularnewline
\hline 
%int.workload & $R^{I}: \{12288 \ CAS \ R, no \ L2WBs, no \ LLCWBs\}$
int. workload & the most permissive workload $k' \in K$ under $D'$
\tabularnewline
\hline 
\hline 
\textbf{Factors} & \textbf{values}
\tabularnewline
\hline 
MBA delay& $d_{i}$ for the i-th interference core \\& $d_i\in D'$, $i \in \{1;2;3\}$
\tabularnewline
\hline 
\hline 
\textbf{Metric} & \textbf{description}
\tabularnewline
\hline 
Memory & critical memory fetching latency in terms of CPU cycles\\fetching&
$L_{k';(d_1,d_2,d_3)}$ \\latency &
%\tabularnewline
%\hline 
%\textbf{Obs. no.} & $30$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


==> Intel-MBA-Assessment ISORC_2022/introduction.tex <==

%\todo[inline]{UNLOCK Marcello}
%\todo[inline]{unLock Gautam}
%\textbf{@ALL} \textbf{Time-sensitive cloud motivations} \newline
%- leverage the cloud advantages as the workload elasticity, performance, maintainability, \newline
%- reliability - fault tolerance, critical task throttling the no critical task. \newline
%- maximizing the average resource utilization (power efficiency)

As seen in Ericson's Computing Fabric  \cite{ericsson}, and railway use case of EU projects such as SECREDAS \cite{gala:railway}, industries are exploring cloud computing and virtualization for hosting safety-critical applications \cite{CINQUE2022315} as clouds support ease of re-usability, maintainability, and reconfiguration while providing workload elasticity and higher availability. Thus, clouds help industries in reducing their running costs and carbon footprint. %Moreover, industries can sell safety-critical operation as a cloud-based service.
Industries can execute existing safety-critical applications without any significant modifications as Virtual Machines (VMs) in a cloud computing environment. These safety-critical VMs must run alongside other non-critical/best-effort VMs executing in the cloud. All VMs are unaware that they are running in a virtualized environment or know the actual underlying cloud nodes or hardware resources, thanks to the virtualization (abstraction) provided by the hypervisor.

Cloud nodes are based on COTS multicore processors, which are rich in shared resources to allow fast communication and improve the average resource utilization. Nevertheless, sharing introduces new forms of non-determinism and dependencies (in space and time) between parallel flows complicating the analysis of the Worst-Case Execution Time (WCET), which is fundamental for safety-critical applications. %In particular, co-executing tasks or VMs add a new circular dependency between the scheduling and WCET analysis; the scheduling uses the WCET to decide on a schedule, while the WCET analysis itself depends on the schedule of the other cores of the same node. \newline

Recent research on real-time hypervisors focused mainly on CPU virtualization, adopting either hierarchical scheduling \cite{RT-XEN_xi2014real} or CPU partitioning \cite{jailhouse}, and implementing cache coloring \cite{modica2018supporting} to reduce inter-core cache interference in multicores. However, open problems regarding temporal contention (and consequent unexpected delays) are still observed when tasks/VMs co-executing on different cores need to access the memory (controller) simultaneously. \newline
Memory access contention deserves special attention for two main reasons: (i) memory accesses are unavoidable, and, contrarily to other sources of temporal contention\cite{Lundqvist1999TimingAI}\cite{Reineke2006ADA}, (ii) memory access interference can increase the WCET by several orders of magnitude, particularly when increasing the number of co-accessing cores \cite{Nowotsch2013, Pellizzoni2010WorstCD}. The picture is even more complex on modern multicore architectures for cloud computing where many cores (or hardware threads) share additional resources such as a Last Level Cache (LLC). For instance, the spatial contention in the LLC has a significant impact on the memory access contention as LLC writebacks lead to asynchronous memory accesses.
While memory accesses are synchronous with respect to the requester demand, asynchronous memory accesses (e.g., due to LLC writebacks) may depend on the memory requests from other cores, as the LLC is shared.

%Therefore, below, we introduce the temporal contention starting from intra-core context moving versus our interest inter-core context. Even if spatial contention is not our main topic, we describe how it is coupled with memory temporal contention.
%Inside a private core context, instructions (ILP) and multiple hardware threads, as a result of simultaneous multi-threading (SMT), contend simultaneously for access to several resources such as functional units and caches, improving private resource utilization. The literature does not still address interference from SMT (e.g., Hyper-threading in Intel processors) as this feature can be easily disabled. \sout{Even if, this feature could be investigated for a deterministic temporal throttling role being a standard feature on modern cloud platforms.}\todo{GG: do we need this sentence; it is grammatically incorrect and I am not sure what you want to say here}
%Contrarily, the contention of functional units between parallel instructions is a well-known source of temporal anomalies \cite{Lundqvist1999TimingAI}\cite{Reineke2006ADA}. It can be handled by several serialization instructions restoring the program order or by increasing the analysis complexity.
%While the intra-core interference can be analyzed or avoided without impacting the overall system utilization, a non-efficient algorithm for inter-core interference affects the entire system performance. 
%On the modern multicore system, several cores (or hardware threads) share several resources such as a last level cache (LLC), network of interconnect and memory.

%\sout{Even though spatial contention is not our main topic,} The spatial contention in the LLC has a significant impact on the memory access contention as LLC writebacks lead to asynchronous memory accesses.
%While synchronous memory accesses are "synchronous" only with the requester demand, these asynchronous memory accesses depend on the memory requests from cores as the LLC is shared.
%This means that temporal memory access partitioning is not possible until we do not have LLC spatial partitioning.
%The main software solution for LLC spatial partitioning is horizontal partitioning leveraging the MMU (Memory Mapping Unit). Even if this solution is configurable on almost any architectures, horizontal partitioning implicitly divides the memory space, and thus, reducing page choices. Hence, special hardware support for cache way-partitioning (vertical partitioning) is favorable, e.g., Intel's Cache Allocation Technology (CAT) \cite{IntelRefManXeonScal}.
%While LLC partitioning allows to identify distinct core flows versus the memory\todo{GG: not clear what you want to say here}, how to regulate these flows continuous is an open question. 

Existing work proposes several memory access regulation methods to limit the maximum interference for the worst case memory access latency analysis.
The basic idea is to limit the memory accesses from individual cores for each regulation period \cite{Yun2013MemGuardMB} \cite{Modica2018SupportingTA}. Thus, it is possible to distribute the available memory access bandwidth and obtain a tighter worst case memory access latency bound.
Software-based resource limitation approaches, such as Memguard \cite{Yun2013MemGuardMB}, require monitoring the memory requests (or cache misses) from each core and applying a throttling policy to prevent memory accesses from cores that have depleted the assigned memory budget for that regulation period.
Despite the design simplicity of software-based approaches, it is not possible to achieve high resolution and efficiency due to the coarse-grained regulation period duration and high overheads. In addition, the throttling policy of the approaches involve stalling the core execution to prevent memory accesses. Such a throttling policy is not suitable for cloud VMs as a core cannot continue its execution within the private context, such as private caches and functional units, reducing the private resources utilization.


A possible way to overcome the limitations of software-based approaches is to rely on 
hardware support. In this respect, Intel recently proposed a new hardware feature known as Memory bandwidth allocation (MBA) present in Xeon Scalable processors \cite{IntelRefManXeonScal}, depicted in Fig. \ref{fig:architecture}. MBA delays the requests going to the interconnect from a core's private context. Intel provides nine values between $10$ to $90$ in increments of $10$ representative of the delays that are inserted between the requests.
%MBA provides nine configurable delays between $10$ to $90$ in increments of $10$, and 
MBA can be used to apply indirect memory bandwidth throttling overcoming the limitations of software base-approaches as: (1) we have a fine-grained regulation period because the delays are inserted by hardware between requests (2) a hardware based method does not require software intervention, except for the initial setup,  to partition memory bandwidth statically  (3) the core execution is not stalled to prevent memory access, thus preserving the private resource utilization.

Despite these promising features, it is still unclear if and how MBA can be used for memory regulation to provide real-time guarantees to safety-critical VMs. As a matter of fact, the MBA controller  does not directly allocate memory bandwidth to cores, and hence the memory bandwidth allocation/regulation is an indirect consequence of the introduced delay.

In this paper, we present the results of a measurement study performed on Intel Xeon Scalable processors in order to derive the indirect memory bandwidth achieved by the cores through MBA for providing real-time guarantees. 
%our main contribution regards the Intel MBA assessment as an indirect memory bandwidth regulation controller for real-time.
The main contributions and results of the study are:
\begin{enumerate}
    \item We propose a systematic approach to derive the indirect memory bandwidth limitation from delay values using a single-core analysis where we highlight the importance to consider also L2 writebacks within the design of experiments;
    \item We experimentally prove that only the 70, 80 and 90 MBA delay values are effective in our setting at limiting the memory bandwidth even in the presence of LLC write-backs (asynchronous memory accesses);
    \item We test the derived assured memory fetching latency for a core allocated to a critical VM when MBA limits the bandwidth of three interfering cores with a multicore analysis, showing the potential and effectiveness of the approach.
    %\item {\color{violet}{We propose a prediction model to interpret the assured bandwidth.}}
\end{enumerate}
The rest of the paper is structured as follows. Section \ref{sec:back} presents the related work, while the background on new Intel MBA feature is provided in Section \ref{sec:intel}. Our design of experiments is presented in Section \ref{sec:doe}, while Sections \ref{sec:one-core-res} and \ref{sec:multi-core-res} presents the results of single-core and multicore analysis, respectively. Finally Section \ref{sec:concl} ends the paper with final remarks and hints for future work.

\begin{figure} 	
	\centering
	\includegraphics[width=0.47\textwidth]{pictures/arch_mba.png}
	\caption{Abstract model of Intel Xeon memory hierarchy depicting the MBA controller between the cores and high-speed interconnect \label{fig:architecture}}
\end{figure}
%\todo[inline]{GG: suggestion for figure 1: make text black so it is easy to read and change color of boxes in black. L1 = \$L1 for making it easy to understand that it is a cache. May be the caption can also be simplified (DONE)}
%\begin{enumerate}
    %\item We describe how to derive the achievable memory bandwidth from a particular delay regarding different sources of variability for a memory load workload. In addition, we investigate the component reliability comparing the variability with and without MBA throttling.
   % \item afterward, we test the critical assured bandwidth in the identified worst-case traffic pattern when the MBA throttles the interference cores.
    %\item in conclusion, we interpret these critical memory bandwidth observations by a predicting model and we conclude our assessment comparing the target MBA with the state of art MemGuard.
%\end{enumerate}




==> Intel-MBA-Assessment ISORC_2022/modeling_multicore_latencies.tex <==
Doubts:
- do we want to propose in this paragraph a predictive model or a model to interpret the data?
- if we want to use a predictive model, we need to show that the model limits the worst case upwards
- as a predictive model we could use the model presented in the paper "Multicore Interference-Sensitive WCET Analysis Leveraging Runtime Resource Capacity Enforcement". For these few combinations of delays it seems to work well! However in the model, it assumes that delay \_i / i is less than or equal to delay \_k / k to have the worst case. However, this is not the case in our case! Probably because we have a mesh.
\todo{MC: I'd rather fuse this section with the previous one and show the model as an intepretation of results}



In this last section, we propose a model to interpret the assured bandwidth easily. 
{\color{red}
L'idea di base è quella di ottenere la banda garantita per un core a partire dai limiti di banda individuati nella one-core analysis insieme a qualche valore di interferenza di riferimento per il modello.
Noi definiamo un grado di interferenza (1 id) del worklaod k come un qualsiasi carico di interferenza equivalente alla massima interferenza generata da un core fisico con il workload k. 
Ad esempio l'unione di più carichi limitati potrebbero essere equivalenti al carico massimo generato da un core fisico.
La nostra approssimazione sta nel considerare l'interferenza generata da più core limitati con l'MBA  come l'unione dei gradi di interferenza individuati nella single-core-analysis.
Ad esempio quando applichiamo un ritardo 90 il grado di interferenza si dimezza, quindi noi approssimiamo l'unione di più carichi ritardati con 90 a un unico carico con un grado di interferenza pari alla somma. 
Quindi interpolando il grado di interferenza al variare del numero di core fisici possiamo ottenere un modello predittivo.
}

The tab.~\ref{sec:fineg_max_BW} describes the results of one-core analysis in terms of decreasing interference degree. Contrarily, tab.~\ref{tab:multicore_combinations_predicted} represents the predicted multicore interference degree when the MBA throttles the three interference cores. It adopts the value of tab.~\ref{sec:fineg_max_BW} as input. 
We use these multicore interference degrees as an ordering reference model for our observed values. \newline
Afterwards, in tab.~\ref{tab:manalysis_interferencedegrees}, we empirically measure the first, the second and the third interference degree varying the number of interference cores. \newline
Our predicting model is built interpolating these observed interference degree of tab.~\ref{tab:manalysis_interferencedegrees}.
The predicted values are obtained by sampling the predicting model latency into the predicted multicore interference degree of tab.~\ref{tab:multicore_combinations_predicted}.
\begin{table}
\caption{Interference degrees: maximum latency in terms of cpu cycles (TSC) when the number of interference cores varies\label{tab:manalysis_interferencedegrees}}
The fig.~\ref{fig:predictting_model_obs_values} shows on the same plot the expected and observed latency values.

\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 0 cores  &1 cores &2 cores &3 cores \\
 & (0 i.d.)  & (1 i.d.) & (2 i.d.) & (3 i.d.)
\tabularnewline
\hline 
\hline 
max latency& 146010 & 220968 & 309222 & 387916 \\
(cpu cycles)&&&&
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{single-core analysis: how the interference degree decreases with a throttling delay \label{sec:fineg_max_BW}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
op. condition & no-thrott & 80-delay & 90-delay
\tabularnewline
\hline 
\hline 
no L2 WB & $id$  & $\approx(3/4)id$ & $\approx(1/2)id$
\tabularnewline
\hline 
\end{tabular}
\end{center}
\end{table}



\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{pictures/predicted_interf_degrees.png}
\caption{Maximum critical latency predicting model. The blues are the empirical measures. The reds are the predicted values. \label{fig:predictting_model}}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{pictures/predicted_interf_degrees_with_observed_values.png}
\caption{Maximum critical latency predicting model. Observed values and expected values. \label{fig:predictting_model_obs_values}}
\end{figure}

==> Intel-MBA-Assessment ISORC_2022/new_Intel_capabilities.tex <==
In this work we focus on the Intel Cascade-Lake micro-architecture, which inherited from the Skylake-Server micro-architecture an exclusive LLC and a mesh as a network of interconnect. An LLC exclusive frees the last level cache to be as large as the sum of all core private caches, saving the private cache size scalability (i.e., we went from 254KB to our 1MB L2 cache size). At the same time, the mesh allows higher parallelism in the memory access and last level cache.  \newline
It is important to take into account the exclusivity property of the LLC when designing the workload for the measurements (see next section). An exclusive LLC does not include all private cache lines, improving the overall cache space utilization. Such property influences the handling in response to an LLC miss where the new fetched cache line is not brought in LLC to keep the inclusivity.\newline
The considered micro-architecture, as well as all the new Intel Xeon processors, supports temporal and spatial isolation at the hardware level through Resource Director Technology (RDT) \cite{IntelRefMan}. We can associate spatial and temporal properties with a class of service (CLOS) and then bind the CLOS to a virtual core. \newline
One physical core cannot change the class of service of another core. However, it can configure the properties of any CLOS. \newline
RDT makes available monitoring and allocation features. \newline
RDT allocation features enable inter-core resource partitioning.
While the Cache Allocation Technology (CAT) and Code and Data Prioritization (CDP) deal with the LLC spatial partitioning, the Memory Bandwidth Allocation (MBA) addresses the temporal memory contention. The MBA controls a configurable delay for requests going to the network of interconnect from the core private context. By configuring such delays, we can apply an indirect limitation in memory access without impacting the use of private resources such as private caches and functional units. Operationally, a MBA delay value can be associate with a class of service (CLOS), e.g., to limit the memory bandwidth of cores hosting non-critical VMs. If two virtual cores of the same physical core have different delays, the larger delay will override the other.
In our case, disabling the Hyper Threading (HP) in the experiments, we have a side effect \cite{IntelRefManXeonScal}; in particular, the non-active hardware threads are assigned to the CLOS0 by default even though they are disabled. Hence, the CLOS0 has not been used. Otherwise, the hidden delay value of the non-active virtual core (the delay value associated with the CLOS0) overrides the MBA delay value of the active virtual machine on the same physical core when the first is higher than the second one.
%Hence, the CLOS0 has not to be used, otherwise the hidden delay value of the non-active virtual core risk override the MBA delay of the active virtual machine.

==> Intel-MBA-Assessment ISORC_2022/notes.tex <==
%8192
\begin{table}
\caption{The maximum rate corresponding to minimum latency (memory requests in $T$). \label{sec:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{d}^{II})$ &6376&6376&6376&6376\\[1pt]
$max(BW_{d}^{II})\%$ &100\%&100\%&100\%&99\%
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{d}^{II})$ &6376&4183&3091&2097\\[1pt]
$max(BW_{d}^{II})\%$ &90\%&52\%&38\%&25\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

[100;100;100;99;90;52;38;25]
[ 51; 51; 51;51;51;50;38;25]
[16048;16048;16048;15834;14474;8366;6160;4168]
[8192;8192;8192;8192;8192;8079;6080;4105]



\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles for 8192 memory Read and 8192 memory write\label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{d}^{II})$ &198210&200704&196132&198230
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{d}^{II})$ &197715&283966&384918&565952
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}






%\begin{table}
%\caption{The maximum rate corresponding to minimum latency (memory requests in $T$). \label{sec:fineg_max_throug_1op}}
%\begin{center}
%\begin{tabular}{ |c| c| c| c| c| c| }
%\hline 
%op.cond. & no-thrott & 70-delay &80-delay & 90-delay
%\tabularnewline
%\hline 
%\hline 
%no L2 WB & & &  & \\max(Reqs/T)& 8192 &8088 & 6076 & 4112\\
%\%BW&\%100&$\approx\%98$&$\approx\%74$&$\approx\%51$ 
%\tabularnewline
%\hline 
%with L2 WB & & &  &\\ max(Reqs/T)& 8192 & 4280 & 3154 & 2131\\
 %\%BW&\%100&$\approx\%50$&$\approx\%38$&$%\approx\%26$ 
%\tabularnewline
%\hline
%\end{tabular}
%\end{center}
%\end{table}

%\textbf{Other possible experiments - one-core analysis}
%\begin{itemize}
   % \item we should repeat the measurements with six channels (easy, just repeat the script)
  %  \item we could measure also the LLC requests as reference bandwidth for a math formula. While the mem changes with the number of channels, the llc bw should be the same.
  %  \item we could propose a math foormula describing the Memory bandiwth throttling though the number of channels and LLC bandiwdth (supoosing that MBA splits perfectly the LLC BW)
%\end{itemize}

%The fig.~\ref{fig:min_lat_no_l2WB} and fig.~\ref{fig:min_lat_with_l2WB} show how the minimum memory fetching latency changes during the two different traffic conditions when a particular MBA delay is applied. \newline
%\begin{figure}
%\centering
%\includegraphics[width=.5\textwidth]{pictures/onecore_opcond0_thrott_var_512KB}\
%\caption{Minimum memory fetching latency without L2 WB\label{fig:min_lat_no_l2WB}}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=.5\textwidth]{pictures/onecore_opcond1_thrott_var_512KB} \
%\caption{Minimum memory fetching latency with L2 WB\label{fig:min_lat_with_l2WB}}
%\end{figure}


%The MBA should act delaying requests going to the network of interconnect regardless of the other cores' behavior. So, by analyzing the throttling without contention, we can design properly the multicore analysis identifying the worst case condition. \newline




\subsection{The maximum available bandwidth}
We are interested in the minimum execution latency to quantify the maximum available bandwidth for an interference core.
We calculate in tab.~\ref{sec:fineg_max_throug_1op} the maximum number of memory reads in $T$ for each traffic condition $tr$ and MBA delay $d$:
\[
max(BW_{d}^{tr})=\frac{T*reqs_{read}}{min(L_{d}^{tr})};  \ T=min(L_{0}^{I}) 
\]
\[reqs_{read}=max(BW_{0}^{I})=8192
\]
Time window $T$ is the minimum execution latency for a core to fetch its 8192 cache lines when the MBA is disabled. \newline
Analyzing the percentages, we observe that 
\begin{itemize}
    \item the bandwidth in the 2nd operational condition for the delays 70, 80, and 90 is halved than the 1st operational condition.
    \item the other delays have no significant impact on the bandwidth limitation.
\end{itemize}
Why does Intel calibrate delays this way? Below, we justify these observations.
\subsubsection{70,80 and 90 delays}
Intel accounts memory write in the available bandwidth solving the write-back problem in the most straightforward and least architecturally expensive way. If our workload includes writing requests also, while the 1st operational condition does not change, the 2nd operational condition has a new worst case. The new worst case for the 2nd operating condition is when both memory read and memory write operations are required for each memory write request. Delaying L2 write-backs, potential memory writes (LLC write-backs) also are delayed\footnote{Note memory writing can be attributed to a particular physical core only if that physical core has its own LLC spatial partition}. Hence, we believe Intel also delays L2 write-backs in the 2nd operational condition preventing potential LLC write-backs. \newline
In conclusion, to prove our intuition, we reproduce in tab.~\ref{tab:onecore_finallatencies_WriteWorkload} and tab.~\ref{tab:onecore_finallatencies_WriteWorkload} the worst case for a memory write workload where each L2 write-back corresponds to one LLC write-back ($L2WBs=CASWrites$) in the 2nd operational condition. 
Note that:
\begin{enumerate}
    \item $max(BW_{R;d}^{I})=max(BW_{W;d}^{I})$ In the 1st operational condition, only memory reads are possible even if our workload includes memory write requests\footnote{memory write request (i.e., Read For Ownership RFO) consists in reading the cache line and updating the value in cache}. 
    \item $max(BW_{R;70:90}^{I})=max(BW_{W;70:90}^{II})$ The memory requests in the 1st or the 2nd operational condition. While in the 1st operational condition, we have only memory reads, in the 2nd, half of them are memory writes.
    \item $max(BW_{R;70:90}^{II})= \frac{max(BW_{W;70:90}^{II})}{2}$ The memory read requests in the 2nd operational condition for 70,80 and 90 delays are halved to prevent memory writes. This regulation choice is pessimistic because L2 write-back does not always cause LLC write-back and therefore writes to memory.
\end{enumerate}
In the multicore analysis, we choose to cover the correctness for the delays where the worst case of memory reads workload also includes the worst case for a memory write workload.
\subsubsection{Insignificant delays} remind that the MBA introduces an indirect memory bandwidth regulation. The delays are significant from requests going to the last level cache. Only a subset of them is also significant for the memory bandwidth. Probably, longer delays could impact too much on the LLC bandwidth regulation. 
\subsection{MBA variability}
MBA has low variability. The latency variability in tab.\ref{tab:onecore_finallatencies} is the same when there isn't throttling and when the MBA is enabled. The range of variability is around two thousand cycles. \newline 
Hence, the MBA is not a new source of variability, increasing its component reliability for a safety-critical context. Several sources explain this variability; however, the main factors are: 
\begin{itemize}
    \item DRAM refresh cycles are periodical. Two measurements can vary at most of two refresh cycles (around 1400 cpu cycles)
    \item Measures accuracy. The serialization instruction overhead is evaluated in our experiments (subsec.~\ref{measuremnt_tool}) with an error margin (around 200 cpu cycles)
\end{itemize}
The precision of MBA delays is surprisly, purticularly for the absence of outliers.
\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles for 8192 memory reads \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R;d}^{I})$ &144216 &144010 & 144494 & 144410\\[1pt]
$max(L_{R;d}^{I})$  &146010 & 146190 & 146468 & 146174
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &147532&147764&147556&149172\\[1pt]
$max(L_{R;d}^{II})$ &149510&149628&149754&150948
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R;d}^{I})$ &144294 & 146058 & 194466 & 287364\\[1pt]
$max(L_{R;d}^{I})$ &146010 & 147568 & 195470 & 288404
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &163376&282352&383132&566966\\[1pt]
$max(L_{R;d}^{II})$ &164708&283406&384116&567730
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{The maximum rate corresponding to minimum latency (memory read requests in $T$). \label{sec:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & & &  & \\
$max(BW_{R;d}^{I})$ &8192 &8192 & 8192 & 8192\\[1pt]
$max(BW_{R;d}^{I})\%$  &100\% &100\% & 100\% & 100\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R;d}^{II})$ &8024&8024&8024&7917\\[1pt]
$max(BW_{R;d}^{II})\%$ &98\%&98\%&98\%&97\%
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{R;d}^{I})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{R;d}^{I})\%$ &100\% &98\%  &74\%  &50\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R;d}^{II})$ &7237&4183&3080&2084\\[1pt]
$max(BW_{R;d}^{II})\%$ &88\%&51\%&38\%&25\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles for 8192 memory Read and 8192 memory write\label{tab:onecore_finallatencies_WriteWorkload}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{W;d}^{II})$ &198210&200704&196132&198230
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{W;d}^{II})$ &197715&283966&384918&565952
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{The maximum rate corresponding to minimum latency (read/write memory requests in $T$). \label{sec:fineg_max_throug_1op_write_workload}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & & &  & \\
$max(BW_{W;d}^{I})$ &8192 &8192 & 8192 & 8192\\[1pt]
$max(BW_{W;d}^{I})\%$  &64\% &64\% & 64\% & 64\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W;d}^{II})$ &2x6376&2x6376&2x6376&2x6376\\[1pt]
$max(BW_{W;d}^{II})\%$ &100\%&100\%&100\%&100\%
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{W;d}^{I})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{W;d}^{I})\%$ &64\% &63\%  &48\%  &33\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W;d}^{II})$ &2x6376&2x4183&2x3091&2x2097\\[1pt]
$max(BW_{W;d}^{II})\%$ &100\%&65\%&49\%&33\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}


























The multicore analysis quantifies the assured bandwidth when the MBA throttles the other cores. \newline
By the one core analysis, we identified two MBA operating conditions respectively when L2 WBs are present or not. This classification helps us to identify the worst case scenario with respect of the particular workload in input when the MBA throttles the interference cores. \newline
The memory load requests in the second operational condition are halved preventing LLC WBs. Hence, whenever in input there is a memory load workload, the worst case is reproduced by executing the interference cores in the first operational condition. \newline Contrarily, when in input there is a full-operational memory write workload, in the second operational condition, an interference core can achieve more bandwidth using the write-back flow. In conclusion, 
\begin{enumerate}
    \item for a memory load workload, an interference core has to be in the first operational condition (no L2WBs)
    \item for a full-operational memory write workload (where each L2WBs corresponds to LLC WBs), the worst case scenario is in the second operational condition including also the worst case for a memory load workload.
\end{enumerate}
Below, we show the worst case scenario for a memory load workload within a quad-core system. The three interference cores perform memory loads in the first operational condition and they are throttled with significant MBA-delays.
In the experiments, all four cores start with empty private caches. In this way:
\begin{enumerate}
\item the interference cores work in the first operating condition of the MBA (no L2 WB)
\item while the critical core emulates a critical task that fills its private caches.
\end{enumerate}
Workload details are listed in tab.~\ref{tab:manalyis_workload_details} 
\begin{table}
\caption{Workload details \label{tab:manalyis_workload_details}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Scope & Initial state  &Memory fetching &Memory loads 
\tabularnewline
\hline 
\hline 
crit. task & L2 empty & 512KB  & 8192 
\tabularnewline
\hline 
interf. task & L2 empty & 768 KB & 12288

\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}
The tab.~\ref{tab:multicore_combinations_observed} shows how the maximum critical workload latency varies when the MBA throttles the cores with 80 and 90 delays. We sort the combinations in ascending order concerning the maximum latency of the critical task. \newline
For each experiment, we captured two hundred observations. \newline
We filter the data considering the number of load operations performed by the critical task (must be 8192) and a multicore synchronization validity test to capture the interference. 
%The maximum latencies respect the interference degree precedence.
\begin{table}
\caption{Critical core latency variability when the three interference cores are throttled by 70, 80 and 90 delay\label{tab:multicore_combinations_observed}}
\begin{center}
\begin{tabular}{  |c| c| c| c| }
\hline 
\#80 delay & \#90 delay & max latency (cpu cycles) 
\tabularnewline
\hline 
\hline 
0&3 & 243208 
\tabularnewline
\hline
1&2 & 260866 
\tabularnewline
\hline
2&1 & 299914 
\tabularnewline
\hline
3&0 & 313040  
\tabularnewline
\hline

\end{tabular}
\end{center}
\end{table}
%\textbf{Other possible experiments - multicore analysis:}
%\begin{itemize}
 %   \item increase the number of interference cores.
 %   \item try as workload interference a memory write workload testing all delays.
%\end{itemize}













\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles  \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R;d}^{I})$ &144216 &144010 & 144494 & 144410\\[1pt]
$max(L_{R;d}^{I})$  &146010 & 146190 & 146468 & 146174
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &147532&147764&147556&149172\\[1pt]
$max(L_{R;d}^{II})$ &149510&149628&149754&150948
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{W;d}^{II})$ &198210&200704&196132&198230
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R;d}^{I})$ &144294 & 146058 & 194466 & 287364\\[1pt]
$max(L_{R;d}^{I})$ &146010 & 147568 & 195470 & 288404
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &163376&282352&383132&566966\\[1pt]
$max(L_{R;d}^{II})$ &164708&283406&384116&567730
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{W;d}^{II})$ &197715&283966&384918&565952
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}






\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles  \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R;d}^{I})$ &144216 &144010 & 144494 & 144410\\[1pt]
$max(L_{R;d}^{I})$  &146010 & 146190 & 146468 & 146174\\[1pt]
$mean(L_{R;d}^{I})$ & 145331 &145306 & 145368 & 145368\\[1pt]
$CI(L_{R;d}^{I})_{99\%}$  & $\pm$181 & $\pm$165 & $\pm$180 & $\pm$154\\[1pt]
$accuracy(L_{R;d}^{I})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &147532&147764&147556&149172\\[1pt]
$max(L_{R;d}^{II})$ &149510&149628&149754&150948\\[1pt]
$mean(L_{R;d}^{II})$ & 148308 &148374 & 148387 & 150071\\[1pt]
$CI(L_{R;d}^{II})_{99\%}$  &$\pm$177 & $\pm$146 & $\pm$223 & $\pm$170\\[1pt]
$accuracy(L_{R;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{W;d}^{II})$ &198210&200704&196132&198230\\[1pt]
$mean(L_{W;d}^{II})$ & 192111 &192802 & 192780 & 193377\\[1pt]
$CI(L_{W;d}^{II})_{99\%}$  &$\pm$931 & $\pm$1020 & $\pm$952 & $\pm$986\\[1pt]
$accuracy(L_{W;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R;d}^{I})$ &144294 & 146058 & 194466 & 287364\\[1pt]
$max(L_{R;d}^{I})$ &146010 & 147568 & 195470 & 288404\\[1pt]
$mean(L_{R;d}^{I})$ & 145316 &146760 & 195137 & 287735\\[1pt]
$CI(L_{R;d}^{I})_{99\%}$  &$\pm$154 & $\pm$128 & $\pm$92 & $\pm$89\\[1pt]
$accuracy(L_{R;d}^{I})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &163376&282352&383132&566966\\[1pt]
$max(L_{R;d}^{II})$ &164708&283406&384116&567730\\[1pt]
$mean(L_{R;d}^{II})$ & 164155 &282745 & 383543 & 567155\\[1pt]
$CI(L_{R;d}^{II})_{99\%}$  &$\pm$127 & $\pm$120 & $\pm$116 & $\pm$71\\[1pt]
$accuracy(L_{R;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{W;d}^{II})$ &197715&283966&384918&565952\\[1pt]
$mean(L_{W;d}^{II})$ & 195011 &282832 & 382700 & 563612\\[1pt]
$CI(L_{W;d}^{II})_{99\%}$  &$\pm$698 & $\pm$188 & $\pm$274 & $\pm$330\\[1pt]
$accuracy(L_{W;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}






%Workload details are listed in tab.~\ref{tab:manalyis_workload_details}.\newline
{\color{blue}{The tab.~\ref{tab:multicore_combinations_observed} shows how the 99-percentile maximum critical workload latency varies when the MBA limits the interference cores with 80 and 90 delays (i.e., in the first row the three cores are limited with 90-delay). Note that we are assuming that the interference does not depend on the core position (i.e., if we limit the core 1 or the core 2 is indifferent).
We sort the combinations in ascending order concerning the maximum latency.}} 
For each experiment, we captured two hundred observations. \newline

%We filter the data considering the number of load operations performed by the critical task (must be 8192) and a multicore synchronization validity test to capture the interference. 

%\begin{table}
%\caption{Workload details \label{tab:manalyis_workload_details}}
%\begin{center}
%\begin{tabular}{ |c| c| c| c| c| }
%\hline 
%Scope & Initial state  &Memory fetching &Memory loads 
%\tabularnewline
%\hline 
%\hline 
%crit. task & L2 empty & 512KB  & 8192 
%\tabularnewline
%\hline 
%interf. task & L2 empty & 768 KB & 12288
%\tabularnewline
%\hline
%\end{tabular}
%\end{center}
%\end{table}


\begin{table}
\caption{Maximum critical latency when the three interference cores are throttled by 80 and 90 delay\label{tab:multicore_combinations_observed}}
\begin{center}
\begin{tabular}{  |c| c| c| c| }
\hline 
\#80 delay & \#90 delay & max latency (cpu cycles) 
\tabularnewline
\hline 
\hline 
0&3 & 243208 
\tabularnewline
\hline
1&2 & 260866 
\tabularnewline
\hline
2&1 & 299914 
\tabularnewline
\hline
3&0 & 313040  
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}






\begin{table}
\caption{Critical core latency variability when the three interference cores are throttled by 80 or 90 delay\label{tab:multicore_combinations_predicted}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
\#70d & \#80d & \#90d & $id$ calculation & resulting $id$ 
\tabularnewline
\hline 
\hline 
0&0&3 & $(0*(3/4)+3*(1/2)$ & $(1.5)id$
\tabularnewline
\hline
0&1&2 & $(1*(3/4)+2*(1/2)$ & $(1.75)id$
\tabularnewline
\hline
0&2&1 & $(2*(3/4)+1*(1/2)$ & $(2)id$
\tabularnewline
\hline
1&0&2 & $(1*(1)+0*(3/4)+2*(1/2)$ & $(2)id$
\tabularnewline
\hline
0&3&0 & $3*(3/4)+(0*(1/2)$ & $(2.25)id$ 
\tabularnewline
\hline
1&1&1 & $(1*(1)+1*(3/4)+1*(1/2)$ & $(2.25)id$
\tabularnewline
\hline
1&2&0 & $(1*(1)+2*(3/4)+0*(1/2)$ & $(2.5)id$
\tabularnewline
\hline
2&0&1 & $(2*(1)+0*(3/4)+1*(1/2)$ & $(2.5)id$
\tabularnewline
\hline
2&1&0 & $(2*(1)+0*(3/4)+1*(1/2)$ & $(2.75)id$
\tabularnewline
\hline
3&0&0 & $(3*(1)+0*(3/4)+0*(1/2)$ & $(3)id$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


==> Intel-MBA-Assessment ISORC_2022/old/copy_singlecore.tex <==
This section describes the single-core analysis results where the main goal was to estimate the indirect limitation of memory bandwidth when the MBA is enabled.
Below, we represent our results for the three workloads $R^{I}, R^{II}, W^{II}$. 
%Our experiments reproduce the first and the second operational condition in this way:
%our workload reads 2048KB in four granes of 512KB where the 1st and 2nd operational conditions are the first and third grane, respectively.
%he first grane is after the dynamic memory flush finding free space in cache, while the third grane is after reading 1MB, probably finding the private cache full being the L2 size of 1 MB. \newline
%Even though we achieve high precision in our measurements,
%the data are filtered like this (validity test):
%\begin{itemize}
%\item the number of last level cache misses must be equal to the number of memory reads ($ LLCmiss = CASreads = 8192$)
%\item in the 1st operational condition, the total L2 write-backs must be equal to zero ($L2WB = 0$)
%\item in the 2nd operational condition, the total L2 write-backs must be equal to the total memory requests ($L2WB = 8192$)
%\end {itemize}
%The numerical values are listed in tab.~\ref{tab:onecore_finallatencies} where the minimum and maximum workload latencies are associated with the respective environmental conditions. 
\subsection{Results representation}
The statistics out of 45 observations are listed in Tab.~\ref{tab:onecore_finallatencies} where 99\% mean confidence intervals are associated with the respective factors giving a degree of confidence of our measures. The accuracy also is always higher than 99\%.  %The mean latency represents well the latency distribution. We observed that the sample mode, mean and median fall in the same range of 100 cycles.
In addition, fig.~\ref{fig:boxplot_lat_onecoreanalysis} shows the boxplots for each experiment and a mean interpolation for the observations of the same workload and different MBA delays.
$L_{k;d}$ is the latency to execute the workload $k$ when the $d$ MBA delay is active. \newline
We are interested in the minimum execution latency to quantify the maximum available bandwidth for an interference core. We estimate this parameter through the observed minimum latency.
We calculate the maximum number of memory operations in $T$ as
\[
max(BW_{k;d})=\frac{T*max(BW_{R^{I};0})}{min(L_{k;d})}; 
\]
where time window $T$  is the minimum execution latency $min(L_{R^{I};0})$ for a core to fetch its 8192 ($max(BW_{R^{I};0})=8192$) cache lines when the MBA is disabled (0-delay). \newline
Tab.~\ref{sec:fineg_max_throug_1op} presents the maximum number of memory accesses in T only for the delays that have an important impact on the relative 0-delay observing the fig.~\ref{fig:boxplot_lat_onecoreanalysis}. In addition, we report also the percentage of synchronous bandwidth as
\[ max(BW_{k;d})\%= \frac{max(BW_{k;d})*100}{max(BW_{R^{I};0})} \]
Note that the synchronous memory bandwidth could be lower than the achievable memory bandwidth where also the memory writes are accounted (i.e., the workload $W^{II}$ achieves $150\%$ of synchronous bandwidth without a significant limitation). In Tab.~\ref{sec:fineg_max_throug_1op}, "2x" indicates double accesses regarding the memory writes.
\subsection{Results interpretation}
Observing the results, we note that:
\begin{enumerate}
    \item $max(BW_{R^{I};d})>max(BW_{R^{II};d})$ the less restrictive limitation for a memory read workload is when there aren't L2 write-backs.
    \item $max(BW_{R^{I};70:90})\approx max(BW_{W^{II};70:90})$ The maximum memory accesses in the 1st and in the 2nd operational condition is approximately the same for 70, 80 and 90 delays.
    \item $max(BW_{R^{II};70:90})\approx \frac{max(BW_{W^{II};70:90})}{2}$ The memory read requests in the 2nd operational condition for 70,80 and 90 delays are halved to prevent memory writes. This regulation choice is pessimistic because L2 write-back does not always cause LLC write-back and therefore writes to memory.
\end{enumerate}
{\color{red}{
The first observation give us an important alert for the future systematic MBA evaluation. When we test the memory bandwidth limitation for read operations, we have to focus our experiments on the first operational condition when there aren't L2 write-backs capturing the most permissive limitation. For instance, if we measure the limitation in terms of memory read requests in one millisecond probably we are considering the second operational condition and we are mistaking!}} \newline
{\color{magenta}{We discovered that even though some delays do not contribute on the indirect memory bandwidth limitation, the delays 70, 80 and 90 have an interesting behaviour. Indeed, they limit and conserve their limitation even if there are memory writes. In particularly, the 80 and 90 delays limit the memory synchronous bandwidth to 75\% and 50\% respectively, while the 70 delay avoids the overload of asynchronous requests halving the synchronous bandwidth in the second operational condition.}} \newline
For these reasons, in the multicore analysis, we choose to evaluate the assured bandwidth when the MBA limits the interference core only with 80 and 90 delays.
%For the insignificant delays remind that the MBA introduces an indirect memory bandwidth regulation. The delays are significant from requests going to the last level cache. Only a subset of them is also significant for the memory bandwidth. Probably, longer delays could impact too much on the LLC bandwidth regulation. 
\subsection{MBA variability}
MBA has low variability. The latency variability as difference between maximum and minimum latency, in tab.\ref{tab:onecore_finallatencies}, is the same (or lower) when there isn't throttling and when the MBA is enabled. Hence, the MBA is not a new source of variability, increasing its component reliability for a safety-critical context.  We tried also other workload size and the range of variability continuous to be around the same. 
The range of variability is around two thousand cycles for a read workload. Several sources explain this variability; however, the main factor are the peridoic DRAM refresh cycles. Two measurements can vary at most of two refresh cycles (around 1400 cpu cycles). The write workload, in addition, has the undisclosed hash function that maps the physical addresses to LLC slices. The structure in slice increases the access variability. \newline
The precision of MBA delays is surprisly, purticularly for the absence of outliers.





\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles  \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R^{I};d})$ &144216 &144010 & 144494 & 144410\\[1pt]
%$max(L_{R^{I};d})$  &146010 & 146190 & 146468 & 146174\\[1pt]
$mean(L_{R^{I};d})$ & 145331 &145306 & 145368 & 145368\\[1pt]
$CI(L_{R^{I};d})_{99\%}$  & $\pm$181 & $\pm$165 & $\pm$180 & $\pm$154
%$accuracy(L_{R^{I};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R^{II};d})$ &147532&147764&147556&149172\\[1pt]
%$max(L_{R^{II};d})$ &149510&149628&149754&150948\\[1pt]
$mean(L_{R^{II};d})$ & 148308 &148374 & 148387 & 150071\\[1pt]
$CI(L_{R^{II};d})_{99\%}$  &$\pm$177 & $\pm$146 & $\pm$223 & $\pm$170
%$accuracy(L_{R^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W^{II};d})$ &187598&185714&187664&187738\\[1pt]
%$max(L_{W^{II};d})$ &198210&200704&196132&198230\\[1pt]
$mean(L_{W^{II};d})$ & 192111 &192802 & 192780 & 193377\\[1pt]
$CI(L_{W^{II};d})_{99\%}$  &$\pm$931 & $\pm$1020 & $\pm$952 & $\pm$986
%$accuracy(L_{W^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R^{I};d})$ &144294 & 146058 & 194466 & 287364\\[1pt]
%$max(L_{R^{I};d})$ &146010 & 147568 & 195470 & 288404\\[1pt]
$mean(L_{R^{I};d})$ & 145316 &146760 & 195137 & 287735\\[1pt]
$CI(L_{R^{I};d})_{99\%}$  &$\pm$154 & $\pm$128 & $\pm$92 & $\pm$89
%$accuracy(L_{R^{I};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R^{II};d})$ &163376&282352&383132&566966\\[1pt]
%$max(L_{R^{II};d})$ &164708&283406&384116&567730\\[1pt]
$mean(L_{R^{II};d})$ & 164155 &282745 & 383543 & 567155\\[1pt]
$CI(L_{R^{II};d})_{99\%}$  &$\pm$127 & $\pm$120 & $\pm$116 & $\pm$71
%$accuracy(L_{R^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W^{II};d})$ &189228&281954&381588&562524\\[1pt]
%$max(L_{W^{II};d})$ &197715&283966&384918&565952\\[1pt]
$mean(L_{W^{II};d})$ & 195011 &282832 & 382700 & 563612\\[1pt]
$CI(L_{W^{II};d})_{99\%}$  &$\pm$698 & $\pm$188 & $\pm$274 & $\pm$330
%$accuracy(L_{W^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{The maximum rate and the percentage of synchronous memory bandwidth corresponding to minimum latency (memory operations in $T$). \label{sec:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{R^{I};d})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{R^{I};d})\%$ &100\% &98\%  &74\%  &50\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R^{II};d})$ &7237&4183&3080&2084\\[1pt]
$max(BW_{R^{II};d})\%$ &88\%&51\%&38\%&25\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W^{II};d})$ &2x6376&2x4183&2x3091&2x2097\\[1pt]
$max(BW_{W^{II};d})\%$ &155\%&101\%&75\%&51\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}
\begin{figure} 	
	\centering
	\includegraphics[width=0.47\textwidth]{pictures/boxplotAlldelaysCols.png}
	\caption{Boxplot latencies for the different workload and interpolation of the respective mean latencies  \label{fig:boxplot_lat_onecoreanalysis}}
\end{figure}









==> Intel-MBA-Assessment ISORC_2022/old/doe.tex <==
\textbf{\todo[inline]{Temporary UNLOCK: TUKL}}
\todo[inline]{GF: we should provide data on the statistical quality of the data, eg, confidence intervals (DONE We put the boxplots avoiding the huge table)}
\todo[inline]{GG: at some point we should mention exactly which processor (name) we used}
Our experiments are composed of two main analysis.
Single core analysis is a systematic approach to deriving the indirect memory bandwidth limitation achieved when the MBA delays the requests. 
Contrarily, the multicore analysis is focused on the guarantees rather than the limitation.
Multicore analysis tests the memory bandwidth achieved by a core executing a critical VM when the MBA (indirectly) limits memory accesses from 3 interfering cores (executing best-effort tasks).
Both, Single-core and multicore analysis, share the following architectural parameters (tab.~\ref{tab:share_parameters}).We use only one socket (one processor) composed of eight cores at most. We set the number of active cores via BIOS configuration. We only used one memory channel in both the analysis. 
%One DRAM channel throughput seems satisfying the core arrival rate. 
%In this architecture, six channels are plugable at most. 
In the BIOS, we set the DRAM refresh rate to periodic and the CPU core frequency to maximum (no power saving). These parameters helped to keep the latency variability to a minimum and maximize the memory requests rate. Similarly, we disabled the Pre-fetcher and Hyperthreading to reduce variability.
Next subsections present the design of experiments for both the analysis.
\begin{table}
\caption{Design of experiments: shared parameters \label{tab:share_parameters}}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
Shared parameters & setting
\tabularnewline
\hline 
\hline 
Socket & 1
\tabularnewline
\hline 
Used DRAM channel & 1
\tabularnewline
\hline 
Prefetcher & disabled 
\tabularnewline
\hline 
SMT &disabled
\tabularnewline
\hline
DRAM refresh cycles & periodic
\tabularnewline
\hline
core frequency &Maximum
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


\subsection{Single-core analysis}
Single-core analysis has to estimate the maximum limitation for an interfering core when MBA is enabled with different delays (As per the Intel errata \cite{IntelRefManXeonScal}, delay values of 20 and 30 are erroneous on our processor and produce the same result as delay value 10).
Our experiments measures the latency execution variability for different kind of workloads.
\subsubsection{Memory read workload}
A read request in the worst case corresponds to a memory read operation when there is a LLC miss. Since we consider this worst case in our workload, read request and memory read operation are interchangeable terms.
However, we identify two different L2 traffic patterns for this worst case as a result of the LLC exclusivity in the processor. \newline
Inclusive and exclusive LLC handle an LLC miss differently. While an inclusive approach holds the new cache line into LLC and L2 keeping the inclusivity  [fig.\ref{llc_handling} (b)], the exclusive one fetches the new cache line only in private cache [fig.\ref{llc_handling} (a)].\newline These distinct approaches entail a different sequence of cache operations when there is a memory read.
In an inclusive architecture, the L2 writeback occurs only when the L2 set is full and the evicted L2 cache line is not updated (dirty) with the LLC copy[fig.\ref{llc_handling} (d)]. 
Therefore, there aren't L2 writebacks when we run only read requests in an inclusive architecture. Contrarily, in the exlusive architecture, we have L2 writeback whenever we read new memory  and the L2 set is full [fig.\ref{llc_handling} (c)]. 
\todo[inline]{GG: do we need to explain all this about inclusive and exclusive architecture or is it enough to explain why exclusive architecture causes 2 different traffic patterns?}
\begin{figure} 	
	\centering
	\includegraphics[width=0.45\textwidth]{pictures/llcmiss_handling.png}
	\caption{LLC miss handling in an inclusive and exclusive architecture respectively when there is space in L2 (a) (b) and when the L2-set is full (c) (d). We suppose available LLC space. \label{llc_handling}}
\end{figure}
The new Xeon processor (and so our micro-architecture) has an exclusive LLC.
Hence, our experiments include the two L2 traffic patterns as a factor. \newline
We prove our intuition in fig.\ref{fig:fineg_l2_wb_00} and fig.\ref{fig:fineg_l2_wb_90} where we fetch 2 MB of dynamic memory in several blocks of 64 KB when the MBA is disabled (0-delay) and enabled with 90-delay. 
While the above plot represents the latency (cpu cycles) for each block, the graph below shows the respective L2-WBs for each fetched block. The number of L2 write-backs grows as the L2 cache fills its capacity (L2 size is 1 MB). While initially L2 capacity is available and so there aren't L2 write-backs, when the L2 becomes full, each memory read sure corresponds to one L2 write-back (so 64KB of memory fetching correspond 1024 L2 write-backs). \newline
Noting the figures, we have two main observations. Without throttling (0-delay), the memory load latency does not change significantly when the L2 write-backs are present (fig.\ref{fig:fineg_l2_wb_00}) because L2 write-backs never cause LLC write-backs for a memory load workload. However the latency changes when the MBA is enabled (fig.\ref{fig:fineg_l2_wb_90}) on the two traffic patterns. The MBA probably  delays the L2 write-back requests. This explanation is entirely plausible because the controller should introduce a delay towards all outgoing requests on the interconnection network, thus also including reads and writes versus the last level cache. \newline
The second observation motivates the choice of consider L2 traffic pattern as a factor. The $R^{I}$ and $R^{II}$ in tab.~\ref{tab:doe_onecoreanalysis} represent respectively the read workload in the first operational condition (without L2 WBs) and in the second operational condition (with L2WBs).
In particularly, the read workload is composed of 8192 read requests where each request is an LLC miss ($ readReqs = LLCmiss = CASreads = 8192$) and hence a memory read operation. In $R^{I}$, the total L2 write-backs must be equal to zero ($L2WB = 0$), while in $R^{II}$, the total L2 write-backs must be equal to the total memory requests ($L2WB = 8192$).
These equalities serve as a validation test.
\subsubsection{Memory write workload}
write requests for a miss cache line in a write-back policy are memory reads operations until a dirty LLC cache line is evicted causing a memory write. Hence, since our write workload reproduces the worst case, every our write request causes one memory read and one memory write operation. The worst case of write requests has only one possible L2 traffic pattern because an LLC write-back is effect of an L2 write-back.
The $W^{II}$ in tab.~\ref{tab:doe_onecoreanalysis} represents this kind of workload.
In particularly, the $W^{II}$ workload is composed of 8192 write requests where each request is cause of one memory read and one memory write ($ writeReqs = LLCmiss = CASreads = CASwrites = 8192$). For the write workload only the second operational condition is possible since an LLC write-back is a consequence of L2 write back.
Agian, these equalities serve as a validation test.
%In conclusion the one-core analysis consists to evaluate the memory fetching latency when the MBA delays and traffic patterns change.
\begin{figure}
\centering
\includegraphics[width=.48\textwidth]{pictures/fineg_mba_thrott_latency_continuous_64KB_memory_fetching_delay0} \
\caption{2048 KB memory fetching in several blocks of 64KB when the MBA is disabled (0-delay)\label{fig:fineg_l2_wb_00}}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=.48\textwidth]{pictures/fineg_mba_thrott_latency_continuous_64KB_memory_fetching_delay9} \
\caption{2048 KB memory fetching in several blocks of 64KB when the MBA 90-delay is enabled\label{fig:fineg_l2_wb_90}}
\end{figure}
\subsection{Multi-core analysis}
While the single-core analysis gives us information about the memory access limitation when the MBA-delay and workload are fixed, the multi-core analysis analyzes the assured bandwidth for a critical core when the MBA limits the other ones. 
In the multi-core analysis, we deploy a quad-core system evaluating how changes the assured bandwidth when there is interference.\newline
In particularly, we consider a specific case where one critical core fetches its dynamic memory without MBA throttling, while the other three cores create interference accessing the memory with maximum rate and they are limited by the MBA. \newline
The range of delays and the particular workload considered for the interference cores will depend on the result of single-core analysis focusing the analysis in the worst-case.In addition, we interpret the observed data thorough a model.
\subsection{Measurement tool and workload considerations \label{measuremnt_tool}}
We performed experiments in Linux as the high server boot duration (several minutes) makes it time consuming to do bare-metal development and experimentation. \newline
%In particularly, we decompose our memory load workload in several configurable blocks focusing our observation on different traffic patterns (Fig.~\ref{exec_model_exp}).
Our measurement tool captures the latency and several factors (such as LLC writeback, L2 writeback and CAS commands) of a particular workload. The latency is captured in terms of TSC (Timestamp counter). The fixed TSC frequency is close to the maximum CPU frequency, hence, we refer to TSC cycles as cpu cycles. We favor the latency rather than bandwidth measurements because the latter requires a regulation period limiting the resolution. \newline
%Below, we describe some considerations that we used for precise experiments in x86:
%\begin{itemize}
   % \item the workload and tool run in kernel space avoiding the context switch for the MSR (Model specific register) access and disabling kernel preemption
   % \item The latency is captured in terms of TSC (Timestamp counter). The fixed TSC frequency is close to the maximum CPU frequency. For these reason, we refer to TSC cycles as cpu cycles.
   % \item we use serialization instructions (as fence) to create independent phase and observation, and to keep the instruction order when necessary (i.e., for reading TSC). The overhead of these instructions have to be not considered in the measurements.
%\end{itemize}
%As shown in fig.~\ref{exec_model_exp}, the experiments are repeated overtime.
%Before the execution, each experiment reproduces memory operations flushing the dynamic memory and so cleaning the cache space. \newline
%In this way, we don't reproduce the memory operations as LLC capacity misses because, in our architecture, reading a dynamic memory bigger than entire cache space is not a sufficient condition to ensure a miss. This is due to the undisclosed hash function that binds physical address and LLC slice. \newline
%\begin{figure} 	
%	\centering
%	\includegraphics[width=0.45\textwidth]{pictures/Observation.png}
%	\caption{Experiment execution model \label{exec_model_exp}}
%\end{figure}
The interference workload is wrote in assembly and consists in only read or write operations (full-loop unrolling). The accessed addresses have a stride 
equals to the cache line size\footnote{Our cache line size is 64 Bytes}. The full loop unrolling of memory requests reproduces the maximum arrival rate and so the maximum interference. Even though the loop unrolling of memory requests increases the code size, we design our experiments controlling the absence of extra LLC misses. \newline
We reproduce the two L2 traffic patterns for a read workload through some initial setup operations. To avoid L2 write-backs and to have memory accesses, we flush the dynamic memory before the workload execution, while to reproduce L2 write-backs for the $R^{II}$ workload, we execute also a pre-read workload to fill the L2 cache. \newline
Contrarily, for the write workload $W^{II}$, we reproduce the worst case executing a pre-workload of write-requests filling the entire cache space of dirty and useless cache-lines. In addition to synchronous memory accesses, the dirty cache lines assure LLC write-back (memory write) whenever there is an LLC eviction.

\begin{table}
\caption{Design of experiments: single-core analysis \label{tab:doe_onecoreanalysis}}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
Goal & Quantify and evaluate the MBA \\ &throttling without memory interference
\tabularnewline
\hline 
\hline 
Parameters & setting
\tabularnewline
\hline 
 cores & 1 
\tabularnewline
\hline 
\hline 
Factors & Values
\tabularnewline
\hline 
MBA & delay $d$, $d\in \{10; 40; 50; 60; 70; 80; 90\}$
\tabularnewline
\hline
workload & \begin{tabular}{ c| c| c }
$R^{I}:$ \{&$R^{II}$: \{ &$W^{II}$: \{ \\8192 CAS R;&8192 CAS R;&8192 CAS R;
\\no L2WBs;&with L2WBs;&with L2WBs;
\\no LLCWBs\}&no LLCWBs\}&with LLCWBs\}
\end{tabular}
\tabularnewline
\hline 
\hline 
Metric & Description
\tabularnewline
\hline 
Latency & memory fetching latency in terms of cpu cycle\\&
\{$L_{R^{I};d}$;$L_{R^{II};d}$;$L_{W^{II};d}$\}
\tabularnewline
\hline
Obs. & $45$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{Design of experiments: multi core analysis}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
Goal & Quantify and explain \\& the critical core assured bandwidth \\& when the MBA limits the interference\\& cores with significant delays
\tabularnewline
\hline 
\hline 
\hline 
Parameters & setting
\tabularnewline
\hline 
 cores & 1 critical core and 3 interference cores
\tabularnewline
\hline 
int.workload & $k \ depends \ on \ the \ single \ core \ analysis$
\tabularnewline
\hline crit. workload & $R^{I}: \{8192 \ CAS \ R, no \ L2WBs, no \ LLCWBs\}$
\tabularnewline
\hline 
\hline 
Factors & Values
\tabularnewline
\hline 
MBA & delay $d_{i={1,2,3}}$ for the i-th interference core \\& $d_i\in \{10;40; 50; 60; 70; 80; 90\}$
\tabularnewline
\hline 
\hline 
Metric & Description
\tabularnewline
\hline 
Latency & critical memory fetching latency in terms of cpu cycle\\&
\{$L_{k;(d_1,d_2,d_3)}$\}
\tabularnewline
\hline 
Obs. & $45$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}




==> Intel-MBA-Assessment ISORC_2022/old/introduction.tex <==

\todo[inline]{lock Marcello}
%\textbf{@ALL} \textbf{Time-sensitive cloud motivations} \newline
%- leverage the cloud advantages as the workload elasticity, performance, maintainability, \newline
%- reliability - fault tolerance, critical task throttling the no critical task. \newline
%- maximizing the average resource utilization (power efficiency)

As seen in Ericson's Computing Fabric  \cite{ericsson}, and railway use case of EU projects such as SECREDAS \cite{gala:railway}, industries are exploring cloud computing for hosting safety-critical applications as clouds support ease of re-usability, maintainability, and reconfiguration while providing workload elasticity and higher availability. Thus, clouds help industries in reducing their running costs and carbon footprint. Moreover, industries can sell safety-critical operation as a cloud-based service.

Industries can execute existing safety-critical applications without any significant modifications as Virtual Machines (VMs) in a cloud computing environment. These safety-critical VMs run must alongside other non-critical/best-effort VMs executing in the cloud. All VMs are unaware that they are running in a virtualized environment or know the actual underlying cloud nodes or hardware resources.

Cloud nodes are composed of COTS multicore processors. Multicore architectures are rich in shared resources adding new forms of non-determinism for safety-critical applications. Even though current resource sharing approaches allow fast communication and improve the average resource utilization, shared resources introduce several dependencies (in space and time) between parallel flows complicating the analysis of the Worst-Case Execution Time (WCET). In particular, co-executing tasks or VMs add a new circular dependency between the scheduling and WCET analysis; the scheduling uses the WCET to decide on a schedule, while the WCET analysis itself depends on the schedule of the other cores of the same node. \newline

This results in clouds being non-deterministic as they do not provide resource allocation guarantees to the VMs.
Contrarily, safety-critical VMs depend on the guaranteed and timely allocation of resources to ensure their end-to-end deadlines are met. 
These uncertainties of current cloud models impedes their adoption in safety-critical domains.

Several existing safety standards adopt the concept of strict spatial and temporal partitioning, such as ARINC 653 specification.
Partitioning reduces analysis complexity and opens the previous circular dependency enabling incremental development and certification (iD\&C) paradigm \cite{4702768}. \newline
Mainly, we can use a three-dimensional space to identify the where contention occurs, and thus, the resolution for that cause of contention:
\begin{itemize}
    \item flows in conflict: what kind of flows are in conflict. Conflicting instructions can be of the same task (in a VM) or of two different tasks (potentially from two different VMs);
    \item kind of contention: what source is contended. Mainly, the sources of contention are the resource storage and resource throughput. 
    \item context: where is the conflict. Principally, shared resources are within a physical intra-core or inter-core context.
\end{itemize}

In this paper, we are interested on the temporal contention, in particularly for the memory (controller) accesses from co-executing tasks/VMs allocated to different hardware cores. Memory access contention has special attention for two main reasons:
\begin{itemize}
    \item Memory accesses are unavoidable.
    \item Considering the worst case memory access latency (the maximum contention) for the memory accesses can increase the WCET by several orders in magnitude, particularly with increase in number of co-accessing cores \cite{Nowotsch2013, Pellizzoni2010WorstCD}.
\end{itemize}

Therefore, below, we introduce the temporal contention starting from intra-core context moving versus our interest inter-core context. Even if spatial contention is not our main topic, we describe how it is coupled with memory temporal contention.
Inside a private core context, instructions (ILP) and multiple hardware threads, as a result of simultaneous multi-threading (SMT), contend simultaneously for access to several resources such as functional units and caches, improving private resource utilization. The literature does not still address interference from SMT (e.g., Hyper-threading in Intel processors) as this feature can be easily disabled. \sout{Even if, this feature could be investigated for a deterministic temporal throttling role being a standard feature on modern cloud platforms.}\todo{GG: do we need this sentence; it is grammatically incorrect and I am not sure what you want to say here}
Contrarily, the contention of functional units between parallel instructions is a well-known source of temporal anomalies \cite{Lundqvist1999TimingAI}\cite{Reineke2006ADA}. It can be handled by several serialization instructions restoring the program order or by increasing the analysis complexity.
While the intra-core interference can be analyzed or avoided without impacting the overall system utilization, a non-efficient algorithm for inter-core interference affects the entire system performance. 
On the modern multicore system, several cores (or hardware threads) share several resources such as a last level cache (LLC), network of interconnect and memory.

\sout{Even though spatial contention is not our main topic,} The spatial contention in the LLC has a significant impact on the memory access contention as LLC writebacks lead to asynchronous memory accesses.
While synchronous memory accesses are "synchronous" only with the requester demand, these asynchronous memory accesses depend on the memory requests from cores as the LLC is shared.
This means that temporal memory access partitioning is not possible until we do not have LLC spatial partitioning.
The main software solution for LLC spatial partitioning is horizontal partitioning leveraging the MMU (Memory Mapping Unit). Even if this solution is configurable on almost any architectures, horizontal partitioning implicitly divides the memory space, and thus, reducing page choices. Hence, special hardware support for cache way-partitioning (vertical partitioning) is favorable, e.g., Intel's Cache Allocation Technology (CAT) \cite{IntelRefManXeonScal}.
While LLC partitioning allows to identify distinct core flows versus the memory\todo{GG: not clear what you want to say here}, how to regulate these flows continuous is an open question. 

Existing work propose several memory access regulation methods to limit the maximum interference for the worst case memory access latency analysis.
\sout{Nowadays, the most suitable approach for temporal partitioning is resource limitation.}
The basic idea is to limit the memory accesses from individual cores for each regulation period. Thus, it is possible to distribute the available memory access bandwidth and obtain a tighter worst case memory access latency bound.
Software-based resource limitation approaches, such as Memguard \cite{Yun2013MemGuardMB}, require monitoring the memory requests from each core and applying a throttling policy to prevent memory accesses from cores that have deleted the assigned memory budget for that regulation period.
Despite the simplicity of design of software-based approaches, it is not possible to achieve high resolution and efficiency as:
\begin{itemize}
    \item The high overhead of the approaches and the possible timer resolution limit the regulation period duration (coarse-grained regulation period) impacting the resolution
    \item The throttling policy of the approaches involve stopping the core execution for preventing memory access.  Such a throttling policy is not suitable for a cloud as a core cannot continue its execution within the private context, such as private caches and functional units, reducing the private resources utilization. \newline 
\end{itemize}

Hardware architectures support only the monitoring synchronous per-core memory accesses through a non-architectural performance monitoring event (independent of the architecture). Since existing approaches leverage performance monitoring counters (PMC), they monitor only synchronous memory requests and do not consider memory accesses from asynchronous write-backs.

Intel proposed a new hardware feature with know as Memory bandwidth allocation (MBA) in its new Xeon processors \cite{IntelRefManXeonScal}. 
The MBA delays the requests going to the interconnect from a core's private context. MBA provides configurable nine delay values between $10$ to $90$ in increments of $10$. We can use to apply indirect memory bandwidth throttling.
This controller overcomes the limitations of software base-approaches: (1) we have a fine-grained regulation period because the delays are inserted by hardware between requests (2) a hardware based based method does not require software intervention except for the initial setup (3) the core execution is not stopped to prevent memory access preserving the private resource utilization.

However, the name, Memory bandwidth allocation (MBA), is misleading. The MBA controller only introduces delays between the core private context and the shared context and does not directly allocate memory bandwidth to cores. The memory bandwidth allocation/regulation is an indirect consequence of the introduced delay. Hence, our evaluation contributes to derive the indirect memory bandwidth achieved by cores for providing real-time guarantees. 
%our main contribution regards the Intel MBA assessment as an indirect memory bandwidth regulation controller for real-time.
Mainly,
\begin{enumerate}
    \item {\color{red}{We propose a systematic approach to derive the indirect memory bandwidth limitation.}}
    \item {\color{magenta}{We experimentally prove that the 70, 80 and 90 MBA delay values limit the memory bandwidth even if there are LLC write-backs (asynchronous memory accesses), while the remaining MBA delay values are not significant.}}
    \item {\color{blue}{We test the assured bandwidth for a core allocated to a critical VM when the MBA limits the bandwidth of three interference cores with three significant MBA delay values.}}
    \item {\color{violet}{We propose a prediction model to interpret the assured bandwidth.}}
\end{enumerate}
\begin{figure} 	
	\centering
	\includegraphics[width=0.47\textwidth]{pictures/architecture.png}
	\caption{Abstract Intel Socket memory hierarchy with MBA  \label{fig:architecture}}
\end{figure}

%\begin{enumerate}
    %\item We describe how to derive the achievable memory bandwidth from a particular delay regarding different sources of variability for a memory load workload. In addition, we investigate the component reliability comparing the variability with and without MBA throttling.
   % \item afterward, we test the critical assured bandwidth in the identified worst-case traffic pattern when the MBA throttles the interference cores.
    %\item in conclusion, we interpret these critical memory bandwidth observations by a predicting model and we conclude our assessment comparing the target MBA with the state of art MemGuard.
%\end{enumerate}




==> Intel-MBA-Assessment ISORC_2022/old/new_Intel_capabilities.tex <==
\todo[inline]{temporary UNLOCK: TUKL}
The technological evolution of Intel server micro-architectures can be summarized by passing from the Broadwell to the Skylake-server architecture\footnote{Note our micro-architecture is a CascadeLake. The CascadeLake inherits the presented Skylake-server arichitectural characteristics.}. \newline
The socket of both is composed of several core private contexts and one shared context.
\begin{itemize}
\item Each private context encloses the core with its private caches (L1 and L2).
\item while all private contexts share and contend the network of interconnect, the last level cache, and the DRAM memory.
\end{itemize}
The main differences are the network of interconnect and the inclusiveness of the last level cache.
\begin{itemize}
\item The new Sky-lake server have a Mesh rather than a Ring. Mesh increases request throughput by scaling with the number of cores.
\todo[inline]{GG: do we need so much history about "technological evolution" of intel architecture or can we start directly from the relevant parts of the Skylake architecture? e.g. RDT and LLC. It seems that we are using quite a lot of space for giving information not directly relevant to the hardware under study}
\item The last level cache in the Skylake-server micro-architectures is not inclusive (exclusive). An LLC exclusive frees the last level cache to be as large as the sum of all core private caches. Since it doesn't need the LLC inclusiveness of all cache lines.  However, usually, it requires a bigger directory that holds (theoretically) the state of all cache lines. \newline 
The exclusive LLC fits the scalability needs of the modern micro-architecture complicating the coherency protocol. 
We can have multiple cores with their larger private cache without increasing LLC space. For example, we went from a 254KB L2 with Broadwell to a 1MB L2 with the SkyLake-server. \newline
The second advantage is the efficiency.
While the cache lines are replicated in the inclusive LLC, the exlusive model enables to keep different cache lines in LLC and in private caches.
\end{itemize}
The new Intel Xeon Scalable processors have a Cascade-Lake or Ice-Lake micro-architecture inheriting all the features presented for the Sckylake Server. \newline
Furthermore, these new Intel processors support temporal and spatial isolation at the hardware level through Resource Director Technology (RDT). We can associate spatial and temporal properties with class of service (CLOS) and then bind the CLOS to a virtual core. \newline
One core cannot change the class of service of another core. However, it can configure the properties of any CLOS. \newline
RDT makes available monitoring and allocation features.
\subsection{RDT monitoring features}
The RDT monitoring features of the RDT do not support interrupt mechanisms. The monitoring data must be read synchronously (polling). \newline
In addition to the service class, we can associate a RID (Resource ID) to each virtual core. \newline
Multiple cores with the same RID correspond from a monitoring perspective to a single resource (RID). \newline
We can monitor a two properties of a RID:
\begin{itemize}
\item the occupancy (in bytes) of the last level cache
\item the outgoing band from the LLC towards the memory (total bandwidth) and the outgoing one towards the local processor memory (internal bandwidth)
\end{itemize}

\subsection{RDT allocation features}
RDT allocation features enables the inter-core resource partitioning.
\subsubsection{CAT and CDP}
The Cache Allocation Technology (CAT) implements a cache way-partitioning at the hardware level of the Last Level Cache.
We can define the number of ways for a class of service (CLOS) through a bitmask (of contiguous bits). This mask can isolate the CLOS cache capacity and still control its overlapping with others. \newline
The CDP (Code and Data Prioritization) extends the functionality of the CAT by specializing it in Data and Code. \newline
With this functionality, a class of service can partition its cache capacity into Data and Code.
\subsubsection{MBA}
The Memory Bandwidth Allocation (MBA) allows to allocate the available physical core memory bandwidth. The MBA controls a configurable delay for requests going to the interconnect network from the core private context. By these delays, we can apply an indirect throttling policy in memory access without impacting the use of private resources. We can associate the MBA delay with a class of service. If two virtual cores of the same physical core have different delays, the larger delay will override the other.

==> Intel-MBA-Assessment ISORC_2022/old/related_work.tex <==
\sout{Memory latency is a well-known source of non-determinism in safety-critical (real-time) applications. Even though a task spends only 10 \% of its life cycle to fetch memory, the execution time can increase by 300 \% in an eight-core system due to worst-case memory interference \cite{Pellizzoni2010WorstCD}.} 
The maximum latency variability can be reduced through memory bank aware partitioning because the memory banks work in parallel.
PALLOC \cite{Yun2014PALLOCDB} enables mapping between the memory pages and the physical banks leveraging the MMU. We can change the bank allocation at run-time. \newline
However, few banks reduce the memory level parallelism (MLP), impacting the average performance. \newline
Even though bank partitioning reduces the latency variability, the temporal contention of upstream resources such as the network of interconnect and memory controller or shared banks remains unmanaged.\newline
Under a worst-case perspective, each access incurs the worst-case interference without a predictable analysis or regulation. Below, we extend the classification of \cite{Kotaba2013MulticoreIR} distinguishing analysis and regulation (partitioning) methods. \newline These two macro-classes respectively know or define the maximum processing element interference. 

\subsection{Analyze the interference \label{sec:anal_interf}}
The idea is to know the maximum number of conflicts through static analysis. Under a worst-case perspective, the first goal is to classify each access for what hierarchy memory level will address. Such analysis gets complicated with shared caches. In \cite{Liang2009TimingAO} each access is first analyzed in the absence of inter-core cache conflicts, and subsequently, a separate inter-core cache conflict analysis refines each classified access. \cite{Chattopadhyay2013ScalableAP} improves the estimation of inter-core cache conflicts combining abstract interpretation and path-sensitive verification (e.g., model checking and symbolic execution). In \cite{Chattopadhyay2010ModelingSC}, \cite{Kelter2011BusAwareMW}, \cite{Chattopadhyay2012AUW} shared cache and bus analysis are combined, applying a TDMA bus arbitration. \newline
Interesting is how \cite{Chattopadhyay2010ModelingSC} resolves the circular dependency between the bus and cache analysis. Indeed, conflicts on the shared resource occur when two tasks overlap over time. However, this requires knowing the lifetime of the tasks. By assuming a compositional architecture, \cite{Chattopadhyay2010ModelingSC} can define a valid initial state and resolve the circular dependency. \newline
These analysis approaches have the following drawbacks: 
\begin{itemize}
\item the computational complexity increases with the number of tasks under analysis.
\item the arbiter is supposed to be deterministic as TDMA. However, on the modern COTS there are more optimization policies
\item there are no independent partitions. The solution validity is straight coupled with tasks under analysis.
\end{itemize}
However, probably, this is the precise-way to achieve the tightest bound estimate. So we believe access classifications suitable within a partition where the tasks under analysis are limited or as hint for the partitioning. \newline

\subsection{Regulate the interference \label{sec:regulate_approaches}}
These approaches handle the interference regulating or serializing the accesses.
\subsubsection{Execution model}
The basic idea of execution models is to split the real-time task into different phases and then enforce a high-level co-scheduling mechanism. \newline
The co-scheduler rules implicitly define the contention degree without relying on low-level arbiters.
The accesses are serialized in several phases, and these phases can be overlapped by co-scheduler achieving a predictable degree of interference. \newline
In \cite{Pellizzoni2011APE}, \cite{Boniol2012DeterministicEM} the co-scheduler implements a TDMA policy. However, a TDMA policy is not scalable with the number of cores. \newline
Pellizzoni \cite{Pellizzoni2011APE} proposes PREM handling the contention of main memory between a single-core and several peripherals. While Boniol\cite{Boniol2012DeterministicEM} extends the concept of the execution model to a multicore platform dividing the execution phase into communication and local execution slices. \newline
The execution models require program or compiler modifications. Boniol \cite{Boniol2012DeterministicEM} also proposes a development process and an automated toolset for the designer to program a sliced architecture.

\subsubsection{Resource limitation}
These approaches make predictable and deterministic the maximum interference limiting the processing element accesses. \newline 
They regulate the interference without modifying or statically analyzing the program. \newline This solution needs a throttling policy to stop the processing element access and a monitoring policy for issued request counting. \newline
The first to perceive the potentiality of performance counters to monitor shared resource accesses has been Bellosa \cite{Bellosa1997ProcessCC}, \cite{Bellosa1999TheTD}. Notably, \cite{Bellosa1997ProcessCC} captures on each PE the only interesting available events such as last-level cache hits and references to extract the LLC misses. The LLC-misses represents the processing element synchronous accesses. \newline
Subsequently, the "LLC misses" are available as a non-architectural event on modern COTS. Yun \cite{Yun2012MemoryAC, Yun2013MemGuardMB} indeed leverages this event to monitor the PE accesses. \newline
As throttling policy, Bellosa \cite{Bellosa1997ProcessCC} inserts idle-loop inside TLB-miss handler, while Yun \cite{Yun2012MemoryAC, Yun2013MemGuardMB} deschedules the task from queue-running tasks.
Bellosa explicitly hints processor constructors to add a programmable delay between load/store operations \cite{Bellosa1997ProcessCC}. \sout{Maybe the Intel MBA is the result of this advice.} \newline
Resource limitation software approach share the following drawbacks:
\begin{itemize}
    \item efficiency: they prevent access to the shared resource forbidding the processing element execution reducing the overall system utilization.
    \item resolution: a software implementation limits the achievable resolution concerning handler sub-routine overhead and timer resolution in the regulation period.
\end{itemize}
%In summary, by limiting the number of PE accesses inside a regulation period, we can define a maximum predictable interference. This prevention algorithm can degrade average performance: the not-consumed PE bandwidth would be lost. 
%So Memguard \cite{Yun2013MemGuardMB}  tries to fill this efficiency gap by defining a reclaimable bandwidth into soft-realtime context. Furthermore, the processing elements are free to execute whenever the assured bandwidth is consumed within the regulation period. \newline
%The second observation is about the policy of throttling. \newline
%Resource limitation software solutions prevent access to the shared resource forbidding the processing element execution reducing the overall system utilization. Furthermore, a software implementation limits the achievable resolution concerning handler sub-routine overhead and timer resolution in the regulation period. \newline

\todo[inline]{GG: I think \cite{Nowotsch2013} is missing}.

==> Intel-MBA-Assessment ISORC_2022/rebuttal.tex <==

\section{Rebuttal ISORC 2022}
The ISORC 2022 rebuttal
period will be between 2022-03-22 and 2022-03-27.

During this time, you will have access to the current state of your
reviews and have the opportunity to submit a response of up to 500
words. Please keep in mind the following during this process:

* The response must focus on any factual errors in the reviews and
any questions posed by the reviewers. It must not provide new
research results or reformulate the presentation. Try to be as
concise and to the point as possible.

* The rebuttal period is an opportunity to react to the reviews, but
not a requirement to do so. Thus, if you feel the reviews are
accurate and the reviewers have not asked any questions, then you do
not have to respond.

* The reviews are as submitted by the PC members, without any
coordination between them. Thus, there may be inconsistencies.
Furthermore, these are not the final versions of the reviews. The
reviews can later be updated to take into account the discussions at
the program committee meeting, and we may find it necessary to
solicit other outside reviews after the rebuttal period.

* The program committee will read your responses carefully and take
this information into account during the discussions. On the other
hand, the program committee will not directly respond to your
responses, either before the program committee meeting or in the
final versions of the reviews.

* Your response will be seen by all PC members who have access to the
discussion of your paper, so please try to be polite and constructive.

The reviews on your paper are attached to this letter. To submit your
response you should log on the EasyChair Web page for ISORC 2022 and
select your submission on the menu.


\subsection{Review 1}
%----------- Overall evaluation -----------
SCORE: 0 (borderline paper) \newline
%----- TEXT:
The authors discuss the effectiveness of the memory bandwidth allocation (MBA) technology available in Xeon Processors with RDT (resource director technologies). They show that only a subset of settings are effective. Moreover, the authors explore the memory bandwidth that can be assured to a single core when other cores interfere with concurrent memory accesses.

The design of experiments proposed in the paper is solid. In the "single-core analysis" the memory bandwidth limitation capabilities of MBA are investigated, whereas in the "multi-core analysis" the capabilities of MBA to guarantee memory bandwidth are explored.

The experiments are very interesting and show the current "state of affairs" concerning the capabilities of MBA in controlling memory contention. 
\newline 
\textbf{Since RDT is still a moving target and differs from generation to generation of RDT compatible Xeon processors I am a little hesitant to recommend to accept the paper for a conference.} 


\newline
For me the results are rather suitable to be discussed in a workshop setting since they might very well be outdated in a few month. For that reason the paper is borderline for me. Even if it is well written and the experiments are extremely well conducted.

\subsection{Review 2}
%----------- Overall evaluation -----------
SCORE: 0 (borderline paper) \newline
%----- TEXT:
The authors analyse multicore processors in respect to bandwidth allocation limits due common memory accesses of different cores which may affect or harm each other. They specifically address Intel's memory bandwidth allocation (MBA) technology and perform different evaluations to demonstrate its abilities and limitations. They present the overall architecture of MBA as well as their evaluation settings and the evaluations.

I like the topic of the paper and think it fits in the scope of ISORC, but I think the paper should be structured more clearly and provide more details: \newline
\begin{itemize}
    \item \textbf{Page 3: "We can asociate spatial and temporal properties with a class of service (CLOS) and then bind the CLOS to a virtual core."
Which properties do you mean? What is the impact a CLOS has to the system?}
    \item In addition, please sketch what the Resource Directir Technology does.
    \item \textbf{You write that you disabled the pre-fetcher as well as Hyperthreading to reduce variability. This is highly abstract. I assume you mean varability with respect to bandwith allocation. Is that right?}
    yes, the hyperthreading can interfere in the access to the memory because the two virtual cores on the same physical core share the available pending requests versus the memory, and the hardware (and softare) pre-fetcher can bring in cache a predictable number of cache lines making the successive requests LLC hits rather than LLC miss.
    Such behavior makes hard to achieve the maximum arrival rates in the single core analysis, furthermore, the hardware pre-fetcher is shared between the cores making difficult also the multi-core analysis.
    \item Table I and II need to be explained. Please try to place them to the next page where the explanations can be found. 
    \item Page 4: Please state in detail the difference of the single-core and the multi-core analysis. From your description, also the single-core analysis takes several cores into account. 
    \item \textbf{Page 4. What do you mean by "The number of observations achieves more than 99\% of accuracy."? Please explain.} The accuracy is calculated as the mean confidence interval calculated with 99\% of confidence divided by the sample mean
    
    \item \textbf{Page 4: What do you mean by "exclusive" and "inclusive" architecture? }
    Inclusive LLC includes all the cache lines holding in private caches. After an LLC miss, in an inclusive LLC the new cache-line is brought both in LLC and private cache keeping the inclusiveness, while in an exclusive LLC the new cache line is brought only in private cache. Hence, being an L2 a private cache as we can see by fig.1, in an exclusive architecture we have an L2 WB whenever the set is full even though the evicted cache-line is clean. Contrarily, in an inclusive LLC, being a copy in LLC, if the new cache-line is clean, the L2 writeback is not necessary. 
    
    \item \textbf{Page 4: What is meant by the "latency (cpu cycles)" exactly? The number of processor cycles to fetch a 64 KB block?} yes, in fig.2 and fig.3 are the processor cycles to fetch 64 KB.
    \item \textbf{Page 4: I assume the delay is measured as percentage. Please define it exactly.}
    As we can see by the Tab. I and II, the MBA delay is configurable value between 10, 20, 30, 40, 50, 60, 70, 80, 90. In our architecture, we don't have the value 20, 30 (as explained in page 4, Single-core Analysis, 4 line, "Intel errata"). 
    \item \textbf{Page 5: "The multicore analysis requires thirty observations to achieve a 99\% accuracy." What does this mean?}
    The accuracy is calculated as the mean confidence interval calculated with 99\% of confidence divided by the sample mean. Thirty observations are sufficient to achieve a 99 \% of accuracy.
    \item \textbf{Page 5: "The number of 8192 requests (meaning 512KB of memory fetching) has been chosen since it assures us to not have L2WBs in RI". How does the 2\^13=8192 requests relate to 512KB of memory?} Each request is a cache line (64 byte) as explained in page 5, Measurement tool and workload considerations, "he workload as consecutive memory operations (full-loop unrolling) and choosing a stride between consecutive accesses equal to the cache line size (our cache line size is 64 Bytes)."
    \item \textbf{Please describe in details the differences and motivation for RI and RII and WII}
    
    \item Chapter V.B: Please introduce more structure: Tell the lessens you learned (e.g. in separate paragraphs) and explain them. 
    \item Page 7: Motivate the "interference degree" in details and provide an example. 

\end{itemize}





\subsection{Review 3}
%----------- Overall evaluation -----------
SCORE: 0 (borderline paper) \newline
%----- TEXT:
Paper Overview:

This paper empirically investigates the novel Memory Bandwidth Allocation (MBA) technology, available on Intel Xeon scalable processors. The main purpose of the investigation is to 1) investigate the indirect limitation of memory bandwidth when MBA delays are applied, and 2) investigate the guaranteed memory bandwidth of a critical core (running highly critical workloads) when the MBA delays the other cores in the multi-core analysis. 

Paper Strengths:

- A novel technology (MBA) is investigated in an important context (mixed-criticality real-time system)
- Paper offers interesting observations

Paper Limitations:

- For the experiment-oriented paper (systematic evaluation as claimed by the authors), it slightly falls below the bar. The investigated workloads are not detailed enough nor justified, and there is no discussion of their limitations to the experiment setup and goals. It is not shown how the investigated delays affect the WCET values of the analyzed workloads, while this is an important aspect for real-time analysis. Also, there is no comparison to the existing approaches (MEMGUARD, etc.) that would show true benefits in real-time oriented experimentation.

- The paper is not easy to follow, there are multiple points where the paper presentation could be improved.

- The paper is motivated in the context of Virtual Machines in cloud computing environment, and safety-critical applications executing on mixed-critical real-time systems. I find it very hard to envision such a system, and the only reference for justifying this setup are the studies [8] and [9] which are more of feasibility studies than the actual motivating use cases. From my reading experience, the safety-critical applications are hardly (or even not) running on mixed-critical cloud systems.

Detailed comments:

Abstract:

It is claimed that the paper adopts a systematic measurement approach on real hardware. However, the representativeness of the investigated workloads is not discussed enough. 

Introduction:

"These safety-critical VMs must" --> Must is a strong word in this context.

"other sources of temporal contention" --> Name those.

"Memory bandwidth allocation (MBA)" --> Memory Bandwidth Allocation (MBA), also fix in the abstract

"software base-approaches" --> software-based approaches

Section II:

"(i) interference estimation" --> this is not quite the management of memory access... although it is not a huge problem.

Section III:

"exclusive LLC ... LLC exclusive" --> not the same, be sure which one is correct.

"processors, supports" --> processors, support

"we have a side effect [10]" --> What side effect? It is not enough to just reference Intel RDT

Section IV

"(tab. I)" --> Table I. Fix this appropriately for all the tables and figures. There are many such inconsistencies.

Table II is inconsistent in the categorization logic. In the first row, you have two columns (Goal) and (QUantify...) which is the description of the goal. Then, you have rows where both columns are distinctive categories. You should make the parent rows bold (e.g. Parameters and setting), and you should also make the goal as a single row single column entry. Or even it can go into the caption of the table so that it does not confuse the reader. 

"The number of observations achieves more than 99% accuracy" --> Should be described more formally. 

"a factor motivating our intuition" --> What intuition? 

"when wrtiebacks" --> when writebacks

"This explanation is plausible" --> This might be possible because...

"The second observation" --> Which is the second observation?

"from fig.2," --> Fig. 2. 

"period of 10 us" --> put microseconds

Section V:

"the latency execution" --> "the latency duration"

Section VII:

"L2 writebeacks" --> "L2 writebacks"

"mehtods" --> "methods"

As a final remark, I would suggest the authors explain in more detail the cache-related concepts such as writebacks, etc., and the investigated memory events considering Fig. 1.




\subsection{Review 4}
%----------- Overall evaluation -----------
SCORE: -2 (reject) \newline
%----- TEXT:
I am a bit irritated of your first sentence in the abstract: "Industries are recently considering the adoption of cloud computing for hosting safety critical applications." I do not believe this is true. Are you proposing that an airplane controller is now running in the cloud?

"given delay values (namely 70, 80 and 90)" what unit are you talking here?

I appreciate the exploration of Intel's MBA for real-time systems. However, I strongly think that writing/talking about safety-critical systems executing in the cloud makes no sense. Sorry, I have to reject that idea.




\section{Rebuttal}

\subsection{Response to questions (R)}
\begin{enumerate}
    \item We agree that the results might vary between different processors, however, we give a systematic method to evaluate the indirect limitation where even the L2 WB are considered as factor for a memory read workload. For this reason, we believe that this paper could be very useful for the real-time research where the memory access contention is still a well-known problem and it is suitable for this conference as supported by one of the reviewer (R2).
    \item yes, the hyperthreading can interfere in the access to the memory because the two virtual cores (on the same physical core) share the available pending requests versus the memory. The hardware (and softare) pre-fetcher can bring in cache a set of cache-lines for each LLC miss. Such behavior makes harder to achieve the maximum arrival rates in the single core analysis, furthermore, the hardware pre-fetcher is shared between the cores making difficult also the multi-core analysis.
    \item 
\end{enumerate}



\subsection{Error (E)}
\begin{enumerate}
    \item The single-core analysis consider only one core into account as we can see in Tab. II where the "core" is set to 1 as parameter. Probably, "Single-core analysis has the objective to estimate the memory access limit for an interfering core when MBA is enabled" confounded the reviewer 2, however, the interfering core represents the subject of the analysis and not a further core.
   
\end{enumerate}


\subsection{Hints (H)}
\begin{enumerate}
    \item I ritardi dell'MBA possono anche variare tra un processore e un altro, tuttavia gli esperimenti dovrebbero seguire il nostro approccio sistematico.
    \item
\end{enumerate}

\subsection{Inconsistences (I)}
\begin{enumerate}
    \item The design of experiments
    \item 
\end{enumerate}


\newpage




\begin{table}
\caption{Rebuttal}
\begin{center}
\begin{tabular}{ |c| c| c |c|}
\hline 
Observations & Reviews & Incons. & Response 
\tabularnewline
\hline 
\hline 
\textbf{+ The DOE are solid} & R1 & & 
\tabularnewline
\hline 
\textbf{+ the experiments are interesting} & R1 & &
\tabularnewline
\hline 
\textbf{+ get the difference between single and multi core analysis} & R1 & &
\tabularnewline
\hline 
\textbf{+ the topic fits in the scope of ISORC} & R2 & &
\tabularnewline
\hline 
\textbf{+ paper offer interesting observations} & R3 & &
\tabularnewline
\hline 
\textbf{+ I appreciate the exploration of Intel’s MBA for real-time 
system} & R4 & &
\tabularnewline
\hline 
- RDT is still a moving target& R1& & 1 (R)
\tabularnewline
\hline 
- the results might vary well be outdated in a few months & R1 & & 1 (R)
\tabularnewline
\hline 
- the paper should be structured more clearly and provide more details & R2 & R1 & 1 (H)
\tabularnewline
\hline 
- it is better for a workshop & R1 & R2 & 1 (R)
\tabularnewline
\hline 
- more details on CLOS and RDT & R2 & & 2 (H)
\tabularnewline
\hline 
- why Pre-fetcher and hyperthreading reduce the variability & R2 & & 2 (R)
\tabularnewline
\hline 
- Tab I and Tab II need to be explained & R2 & & 3 (H)
\tabularnewline
\hline 
- single-cores takes several cores into account (page 4) & R2 & R1 & 1 (E)
\tabularnewline
\hline 
- 99\% of accuracy & R2, R3 & & 4(H)
\tabularnewline
\hline 
- explain exclusive and inclusive architecture & R2 & & 5 (H)
\tabularnewline
\hline 
- page 4, latency cpu cycles, 64 KB? & R2 & & 3 (R)
\tabularnewline
\hline 
- MBA delay in percentage? & R2 R4 & & 5 (H)
\tabularnewline
\hline 
- How does the 2ˆ13=8192 requests relate to 512KB of memory & R2 & & 2 (E)
\tabularnewline
\hline 
- more details about the worklaods & R2, R3 & & 6 (H) 
\tabularnewline
\hline 
- interference degree example & R2 & & 3 (E)
\tabularnewline
\hline 
- no experiment setup and details & R3 & & 4 (I)
\tabularnewline
\hline 
- how the delays affect the WCET analysis & R3 & &
\tabularnewline
\hline 
- no comparison to Memguard & R3 & &
\tabularnewline
\hline 
- not easy to follow & R3 & &
\tabularnewline
\hline 
- Safety critical and RT-Cloud & R3, R4 & &
\tabularnewline
\hline 
\end{tabular}
\end{center}
\end{table}

==> Intel-MBA-Assessment ISORC_2022/related_work.tex <==
%\sout{Memory latency is a well-known source of non-determinism in safety-critical (real-time) applications. Even though a task spends only 10 \% of its life cycle to fetch memory, the execution time can increase by 300 \% in an eight-core system due to worst-case memory interference \cite{Pellizzoni2010WorstCD}.} 
%The maximum latency variability can be reduced through memory bank aware partitioning because the memory banks work in parallel.
%PALLOC \cite{Yun2014PALLOCDB} enables mapping between the memory pages and the physical banks leveraging the MMU. We can change the bank allocation at run-time. \newline
%However, few banks reduce the memory level parallelism (MLP), impacting the average performance. \newline
%Even though bank partitioning reduces the latency variability, the temporal contention of upstream resources such as the network of interconnect and memory controller or shared banks remains unmanaged.\newline
%Under a worst-case perspective, each access incurs the worst-case interference without a predictable analysis or regulation. Below, we extend the classification of \cite{Kotaba2013MulticoreIR} distinguishing analysis and regulation (partitioning) methods. \newline These two macro-classes respectively know or define the maximum processing element interference. 

The management of memory access time interference can be broadly classified in two approaches (extending the classification in \cite{Kotaba2013MulticoreIR}): (i) interference estimation, to take it into account in worst case execution time analysis, and (ii) interference regulation by either enforcing execution models or limiting the access to the memory controller at runtime. In the following we review the literature falling into these two categories.

\subsection{Interference Estimation Approaches\label{sec:anal_interf}}
The idea is to analytically estimate the maximum number of conflicts through static analysis. Under a worst-case perspective, the first goal is to classify accesses depending on the addressed hierarchical memory level. Such analysis gets complicated with shared caches. In \cite{Liang2009TimingAO} each access is first analyzed in the absence of inter-core cache conflicts, and subsequently, a separate inter-core cache conflict analysis refines each classified access. \cite{Chattopadhyay2013ScalableAP} improves the estimation of inter-core cache conflicts combining abstract interpretation and path-sensitive verification (e.g., model checking and symbolic execution). In \cite{Chattopadhyay2010ModelingSC}, \cite{Kelter2011BusAwareMW}, \cite{Chattopadhyay2012AUW} shared cache and bus analysis are combined, applying a time-division bus arbitration. \newline
%Interesting is how \cite{Chattopadhyay2010ModelingSC} resolves the circular dependency between the bus and cache analysis. Indeed, conflicts on the shared resource occur when two tasks overlap over time. However, this requires knowing the lifetime of the tasks. By assuming a compositional architecture, \cite{Chattopadhyay2010ModelingSC} can define a valid initial state and resolve the circular dependency. \newline
Estimation approaches suffer from several drawbacks. 
First, the computational complexity increases with the number of tasks.
Second, the arbiter is supposed to be deterministic, enabling time-division multiple access (TDMA). However, this is not possible on modern COTS due to their optimization policies. Third, there are no independent partitions: the estimation validity is stictly coupled with the tasks under analysis.

%However, probably, this is the precise-way to achieve the tightest bound estimate. So we believe access classifications suitable within a partition where the tasks under analysis are limited or as hint for the partitioning. \newline

\subsection{Interference Regulation Approaches \label{sec:regulate_approaches}}
%These approaches handle the interference regulating or serializing the accesses.
\subsubsection{Approaches based on execution models}
The basic idea of execution models is to split real-time tasks into different phases and then enforce a high-level co-scheduling mechanism. 
The co-scheduler rules implicitly define the contention degree without relying on low-level arbiters.
The memory accesses are then serialized in several phases, and these phases can be overlapped by the co-scheduler achieving a predictable degree of interference. 
In \cite{Pellizzoni2011APE}, \cite{Boniol2012DeterministicEM} the co-scheduler implements a TDMA policy. In particular, 
the work in \cite{Pellizzoni2011APE} proposes PREM handling the contention of main memory between a single-core and several peripherals. Whereas, the work in \cite{Boniol2012DeterministicEM} extends the concept of the execution model to a multicore platform dividing the execution phase into communication and local execution slices. \newline
Execution models are invasive, as they require program or compiler modifications. Moreover, the TDMA policy is not scalable with the number of cores. %\newlineBoniol \cite{Boniol2012DeterministicEM} also proposes a development process and an automated toolset for the designer to program a sliced architecture.


\subsubsection{Approaches based on resource limitation}
The aim of these approaches is to make the maximum interference  predictable and deterministc, by limiting the processing element accesses, with no modification to the original program. These solutions are usually based on a throttling policy to stop the processing element access in case of excessive request, and a monitoring policy for counting the issued requests. \newline
Notably, \cite{Bellosa1999TheTD} are among the first ones to perceive the potentiality of performance counters to monitor shared resource accesses. The idea is to capture on each processing element (PE) the only interesting available events, such as last-level cache hits and references to extract the number of LLC misses (representing synchronous accesses). Nowadays, LLC misses are supported as non-architectural events on modern COTS and are also used to monitor PE accesses, \cite{Yun2012MemoryAC, Yun2013MemGuardMB}. \newline
As throttling policy, \cite{Bellosa1997ProcessCC} inserts idle-loops inside TLB-miss handler, while the works in \cite{Yun2012MemoryAC, Yun2013MemGuardMB} propose to deschedule the task.
The work in \cite{Nowotsch2013} starts from the computation of the \textit{interference-sentitive} WCET taking into account a safety bound for shared-resource interference when at runtime resource capacity enforcement is used to limit the actual resource usage of each process, which are executed following a round robin scheduling scheme. Such pessimistic model is based on a strong assumption on the interference delays. \newline
As software-based resource limitation approaches present the already mentioned efficiency and resolution issues, in the rest of the paper we focus on the new capabilities offered by Intel's MBA technology.
%\todo[inline]{GG: we have mentioned quite a bit about software based approaches and their limitations in introduction as well. May be we can shorten it there? (DONE)}
%In summary, by limiting the number of PE accesses inside a regulation period, we can define a maximum predictable interference. This prevention algorithm can degrade average performance: the not-consumed PE bandwidth would be lost. 
%So Memguard \cite{Yun2013MemGuardMB}  tries to fill this efficiency gap by defining a reclaimable bandwidth into soft-realtime context. Furthermore, the processing elements are free to execute whenever the assured bandwidth is consumed within the regulation period. \newline
%The second observation is about the policy of throttling. \newline
%Resource limitation software solutions prevent access to the shared resource forbidding the processing element execution reducing the overall system utilization. Furthermore, a software implementation limits the achievable resolution concerning handler sub-routine overhead and timer resolution in the regulation period. \newline

%\todo[inline]{GG: I think \cite{Nowotsch2013} is missing}.

==> Intel-MBA-Assessment ISORC_2022/results_multi_core_analysis.tex <==
While the single-core analysis focused on the memory bandwidth limitation, we analyze the guaranteed bandwidth of a critical core when the MBA throttles the other cores in the multi-core analysis. \newline
We analyze the delays that significantly limit the synchronous memory bandwidth: 80 and 90 delays reduce synchronous bandwidth by 75 and 50 percent, respectively. In addition, we design an interpretative model to explain the observed data. \newline
We choose $R^{I}$ as interfering workload, as motivated by the single-core analysis results. In the experiments, we deploy a quad-core system where all four cores start with empty private caches. In this way, the interference cores reproduce the $R^{I}$ workload, while the critical core emulates a critical task that fills its private caches. In particular, the critical task fetches 512KB, while the interference cores 768KB, to be sure to last longer than the critical task. \newline
In Table \ref{tab:multicore_combinations_predicted}, we associate an interference degree $id$ to each experiment combination considering the limitation calculated in the single-core analysis.\footnote{Note that we are assuming the combinations position-independent (i.e., if we limit core 1 memory accesses, we suppose to be the same of limiting the core 2).} An interference degree, for us, represents the synchronous memory accesses that we would execute without interference. If that load equals the number of requests performed by a single-core with a maximum rate, then the interference degree is equivalent to one. \newline
The interference degree considers only the limitation of the single-core analysis and not the observed interference. Hence, for instance, the third combination of Table \ref{tab:multicore_combinations_predicted}, where two cores interfere with 80-delays (75\% of synch. bandwidth) and one core with 90-delay (50\% of synch. bandwidth), has the same interference degree of two cores that interfere without limitation.
In Fig. \ref{fig:predictting_model}, we report the boxplots of our critical latency observations for each combination of interference degrees in Table \ref{tab:multicore_combinations_predicted}, and we interpolate the 95-percentile. As expected, the lower the interference degree (achieved with high MBA delays) the lower the impact on the latency of the critical workload. 
\newline
To better interpret this result, we also report the interpolation of the 95-percentile of the critical core latency when having exactly 1, 2 or 3 interfering cores with 0-delay, that is, no MBA limitation (blue line of Fig.~\ref{fig:predictting_model}).

Comparing the two 95-percentile interpolations, we can see how the MBA is effective at limiting the interference. For instance, when the interference degree is set to 2 (with 1 interfering core with 90-delay and 2 interfering cores with 80-delay) the MBA is able to reduce the interference of 3 cores to at most the one we would have with 2 interference cores running without limitation. The blue line can thus be seen as the worst-case memory access latency we can achieve, when varying the interference degree, which is useful to establish a predictable behavior of the critical workload when run in a cloud system. This worst-case line is also easily achievable, from a practical point of view, by running interfering workloads with an increasing number of cores with no MBA. \newline
Hence, our experiments show that the MBA can provide several safety upper bounds for the memory fetching phase of a critical task in a mixed-criticality Cloud infrastructure.Such bounds can be used in the WCET analysis of real-time tasks, without requiring invasive interventions to task code or execution.
%The critical core can restrict the memory access limitation for such phase by varying the delays associated with the class of service (CLOS) of the non-critical tasks. 
%Such limitation is obtained saving as much as possible the non-critical task properties. 
In particular, this solution doesn't require to modify the program of non-critical task to respect execution models (contrarily to \cite{Pellizzoni2011APE}, \cite{Boniol2012DeterministicEM}) and it preserves private resource utilization limiting only the access versus the shared context (contrarily to software solutions such as Memguard \cite{Yun2013MemGuardMB} which halt the core execution).
%have a way to interpret the observed data: \newline
%{\color{blue}{

%In conclusion, the multi-core analysis tested the critical bandwidth for significant MBA limitation values and provided a model to explain the observations showing the potential and effectiveness of the MBA approach.}}


\begin{table}
\caption{Critical core latency variability when the three interference cores are throttled by 80 or 90 delay\label{tab:multicore_combinations_predicted}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
\textbf{ \#80d} & \textbf{\#90d }&\textbf{interference degree $id$ \textbf{calculation}} & \textbf{resulting $id$ }
\tabularnewline
\hline 
\hline 
0&3 & $(0*(3/4)+3*(1/2)$ & $1.5$
\tabularnewline
\hline
1&2 & $(1*(3/4)+2*(1/2)$ & $1.75$
\tabularnewline
\hline
2&1 & $(2*(3/4)+1*(1/2)$ & $2$
\tabularnewline
\hline
3&0 & $(3*(3/4)+0*(1/2)$ & $2.25$ 
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{pictures/InterpretativeModel.png}
\caption{Comparison between the critical execution latencies of the interpretative model and those observed as the degree of interference varies
%as the 95-percentile interpolation of critical latencies when the number of interference cores varies; the boxplots and 95-percentile interpolation of the observed latencies of the critical workload as a function of combinations (interference degree) in Table \ref{tab:multicore_combinations_predicted}  
\label{fig:predictting_model}}
\end{figure}


==> Intel-MBA-Assessment ISORC_2022/results_one_core_analysis.tex <==
This section describes the single-core analysis results where the main goal was to estimate the indirect limitation of memory bandwidth when the MBA is enabled.
Below, we represent our results for the three workloads $R^{I}, R^{II}, W^{II}$. 
 
\subsection{Results representation}
$L_{k;d}$ is the execution latency of the workload $k$ when the $d$ MBA delay is active. \newline
Fig.~\ref{fig:boxplot_lat_onecoreanalysis} shows the $L_{k;d}$ boxplots for each experiment of Table \ref{tab:doe_onecoreanalysis} and a mean interpolation for the observations of the same workload and different MBA delays. \newline
Observing the boxplot width, the latency variability is the same (or lower) when the limitation is enabled or not (0-delay). 
%That variability is tight compared to the mean latencies achieving a high level of accuracy (higher than 99\%) in our measurements. 
Hence, the MBA seems to be not a new source of variability. The main source of that variability is the periodic DRAM refresh cycles.

\subsection{Results interpretation}
The Fig.~\ref{fig:boxplot_lat_onecoreanalysis} shows two effects clearly. The first is that the limitations have not an important impact on the relative 0-delay observations until the 70-delay in our setting. The second is that the boxplots of workload $R^{II}$ and $W^{II}$ overlap for high delays, meaning a similar behavior due to L2WBs. 
\newline
To better interpret the results from Fig.~\ref{fig:boxplot_lat_onecoreanalysis} for the 70, 80, and 90 delays, we prefer to go from the latency to bandwidth domain. \newline
%Assuming the maximum achievable synchronous bandwidth be the total number of read operations we set ($max(BW_{R^{I};0})$=8192), and assuming $T$ to be the minimum execution latency $min(L_{R^{I};0})$ in CPU cycles for a core to perform such $max(BW_{R^{I};0})$ operations, 
Being $T$ the minimum execution latency  $min(L_{R^{I};0})$ to synchronously fetch 8192 cache lines (our chosen reference, as explained earlier),
we calculate the achievable bandwidth (memory operations in $T$) of a generic configuration ${k;d}$, where $k$ is the workload, and $d$ is the delay, as: 
\[
BW_{k;d}=\frac{T*8192}{L_{k;d}}; 
\]
%that is, $BW_{k;d}$ is a fraction of the best case (8192), which is diminished by the latency introduced by the MBA delay.
 We report in Table \ref{tab:fineg_max_throug_1op} the maximum observed bandwidth for delays from 60 to 90. \newline
We evaluate also the maximum percentage of synchronous bandwidth as
\[ max(BW_{k;d})\%= \frac{max(BW_{k;d})*100}{8192} \]
Note that the synchronous memory bandwidth could be lower than the achievable memory bandwidth as also memory writes are accounted (i.e., the workload $W^{II}$ achieves $155\%$ of synchronous bandwidth with the less restrictive 60-delay limitation). This is due to the fact that, in the worst case set by our write workload, each write request causes one memory read and one memory write operation, due to the eviction. The "2x" in Table \ref{tab:fineg_max_throug_1op} accounts for this double access regarding memory writes. \newline
Observing the results in the table, we can note that:
\begin{equation}{max(BW_{R^{I};d})>max(BW_{R^{II};d})}\end{equation} 
hence, the less restrictive limitation for a memory read workload is when there are no L2 writebacks, confirming what anticipated in the previous section. We can also note that:
\begin{equation}{
max(BW_{R^{I};70:90})\approx max(BW_{W^{II};70:90})
}
\end{equation} 
that is, the maximum memory accesses in the 1st and in the 2nd operational condition with writes is approximately the same for 70, 80 and 90 delays. Finally, we can note that: 
\begin{equation}
max(BW_{R^{II};70:90})\approx \frac{max(BW_{W^{II};70:90})}{2}
\end{equation} meaning that the memory read requests in the 2nd operational condition for 70,80 and 90 delays are halved due to L2WBs. This regulation choice is pessimistic because L2 writebacks does not always cause LLC writebacks and therefore writes to memory.

The results confirm an important hint for systematic MBA evaluation. When testing the memory bandwidth limitation for read operations, it is necessary to run  measurements without L2 writebacks (first operational condition) capturing the most permissive limitation.  %For instance, if we measure the limitation in terms of memory read requests in one millisecond probably we are considering the second operational condition, and we are mistaking!}} \newline
\begin{figure} 	
	\centering
	\includegraphics[width=0.47\textwidth]{pictures/boxplotAlldelaysCols.png}
	\caption{Boxplot latencies for the different workloads and interpolation of the respective mean latencies  \label{fig:boxplot_lat_onecoreanalysis}}
\end{figure}
\begin{table}
\caption{The maximum rate and the percentage of synchronous memory bandwidth corresponding to minimum latency (memory operations in $T$). \label{tab:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
\textbf{Metrics} & \textbf{60-delay}&\textbf{70-dela}y &\textbf{80-delay} & \textbf{90-delay} 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{R^{I};d})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{R^{I};d})\%$ &100\% &98\%  &74\%  &50\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R^{II};d})$ &7237&4183&3080&2084\\[1pt]
$max(BW_{R^{II};d})\%$ &88\%&51\%&38\%&25\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W^{II};d})$ &2x6376&2x4183&2x3091&2x2097\\[1pt]
$max(BW_{W^{II};d})\%$ &155\%&101\%&75\%&51\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}
In addition, we discovered that even though some delays do not contribute to the indirect memory bandwidth limitation in our setting, the delays 70, 80, and 90 have interesting behavior. Indeed, they limit and conserve their limitation even if there are memory writes. In particular, the 80 and 90 delays limit the synchronous memory bandwidth to 75\% and 50\%, respectively. In contrast, the 70 delay only avoids the overload of asynchronous requests due to L2WBs, halving the synchronous bandwidth in the second operational condition. \newline These are important aspects to be considered when dimensioning a system with MBA in order to assure a given memory bandwidth to a critical core. \newline
Along this direction, in the multicore analysis, we choose to evaluate the assured bandwidth when the MBA limits the interference workloads $R^{I}$  only with 80 and 90 delays, covering the significant cases of synchronous bandwidth limitation.
%For the insignificant delays remind that the MBA introduces an indirect memory bandwidth regulation. The delays are significant from requests going to the last level cache. Only a subset of them is also significant for the memory bandwidth. Probably, longer delays could impact too much on the LLC bandwidth regulation. 













==> modeling_multicore_latencies.tex <==
Doubts:
- do we want to propose in this paragraph a predictive model or a model to interpret the data?
- if we want to use a predictive model, we need to show that the model limits the worst case upwards
- as a predictive model we could use the model presented in the paper "Multicore Interference-Sensitive WCET Analysis Leveraging Runtime Resource Capacity Enforcement". For these few combinations of delays it seems to work well! However in the model, it assumes that delay \_i / i is less than or equal to delay \_k / k to have the worst case. However, this is not the case in our case! Probably because we have a mesh.
\todo{MC: I'd rather fuse this section with the previous one and show the model as an intepretation of results}



In this last section, we propose a model to interpret the assured bandwidth easily. 
{\color{red}
L'idea di base è quella di ottenere la banda garantita per un core a partire dai limiti di banda individuati nella one-core analysis insieme a qualche valore di interferenza di riferimento per il modello.
Noi definiamo un grado di interferenza (1 id) del worklaod k come un qualsiasi carico di interferenza equivalente alla massima interferenza generata da un core fisico con il workload k. 
Ad esempio l'unione di più carichi limitati potrebbero essere equivalenti al carico massimo generato da un core fisico.
La nostra approssimazione sta nel considerare l'interferenza generata da più core limitati con l'MBA  come l'unione dei gradi di interferenza individuati nella single-core-analysis.
Ad esempio quando applichiamo un ritardo 90 il grado di interferenza si dimezza, quindi noi approssimiamo l'unione di più carichi ritardati con 90 a un unico carico con un grado di interferenza pari alla somma. 
Quindi interpolando il grado di interferenza al variare del numero di core fisici possiamo ottenere un modello predittivo.
}

The tab.~\ref{sec:fineg_max_BW} describes the results of one-core analysis in terms of decreasing interference degree. Contrarily, tab.~\ref{tab:multicore_combinations_predicted} represents the predicted multicore interference degree when the MBA throttles the three interference cores. It adopts the value of tab.~\ref{sec:fineg_max_BW} as input. 
We use these multicore interference degrees as an ordering reference model for our observed values. \newline
Afterwards, in tab.~\ref{tab:manalysis_interferencedegrees}, we empirically measure the first, the second and the third interference degree varying the number of interference cores. \newline
Our predicting model is built interpolating these observed interference degree of tab.~\ref{tab:manalysis_interferencedegrees}.
The predicted values are obtained by sampling the predicting model latency into the predicted multicore interference degree of tab.~\ref{tab:multicore_combinations_predicted}.
\begin{table}
\caption{Interference degrees: maximum latency in terms of cpu cycles (TSC) when the number of interference cores varies\label{tab:manalysis_interferencedegrees}}
The fig.~\ref{fig:predictting_model_obs_values} shows on the same plot the expected and observed latency values.

\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 0 cores  &1 cores &2 cores &3 cores \\
 & (0 i.d.)  & (1 i.d.) & (2 i.d.) & (3 i.d.)
\tabularnewline
\hline 
\hline 
max latency& 146010 & 220968 & 309222 & 387916 \\
(cpu cycles)&&&&
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{single-core analysis: how the interference degree decreases with a throttling delay \label{sec:fineg_max_BW}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
op. condition & no-thrott & 80-delay & 90-delay
\tabularnewline
\hline 
\hline 
no L2 WB & $id$  & $\approx(3/4)id$ & $\approx(1/2)id$
\tabularnewline
\hline 
\end{tabular}
\end{center}
\end{table}



\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{pictures/predicted_interf_degrees.png}
\caption{Maximum critical latency predicting model. The blues are the empirical measures. The reds are the predicted values. \label{fig:predictting_model}}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{pictures/predicted_interf_degrees_with_observed_values.png}
\caption{Maximum critical latency predicting model. Observed values and expected values. \label{fig:predictting_model_obs_values}}
\end{figure}

==> notes.tex <==
%8192
\begin{table}
\caption{The maximum rate corresponding to minimum latency (memory requests in $T$). \label{sec:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{d}^{II})$ &6376&6376&6376&6376\\[1pt]
$max(BW_{d}^{II})\%$ &100\%&100\%&100\%&99\%
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{d}^{II})$ &6376&4183&3091&2097\\[1pt]
$max(BW_{d}^{II})\%$ &90\%&52\%&38\%&25\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

[100;100;100;99;90;52;38;25]
[ 51; 51; 51;51;51;50;38;25]
[16048;16048;16048;15834;14474;8366;6160;4168]
[8192;8192;8192;8192;8192;8079;6080;4105]



\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles for 8192 memory Read and 8192 memory write\label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{d}^{II})$ &198210&200704&196132&198230
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{d}^{II})$ &197715&283966&384918&565952
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}






%\begin{table}
%\caption{The maximum rate corresponding to minimum latency (memory requests in $T$). \label{sec:fineg_max_throug_1op}}
%\begin{center}
%\begin{tabular}{ |c| c| c| c| c| c| }
%\hline 
%op.cond. & no-thrott & 70-delay &80-delay & 90-delay
%\tabularnewline
%\hline 
%\hline 
%no L2 WB & & &  & \\max(Reqs/T)& 8192 &8088 & 6076 & 4112\\
%\%BW&\%100&$\approx\%98$&$\approx\%74$&$\approx\%51$ 
%\tabularnewline
%\hline 
%with L2 WB & & &  &\\ max(Reqs/T)& 8192 & 4280 & 3154 & 2131\\
 %\%BW&\%100&$\approx\%50$&$\approx\%38$&$%\approx\%26$ 
%\tabularnewline
%\hline
%\end{tabular}
%\end{center}
%\end{table}

%\textbf{Other possible experiments - one-core analysis}
%\begin{itemize}
   % \item we should repeat the measurements with six channels (easy, just repeat the script)
  %  \item we could measure also the LLC requests as reference bandwidth for a math formula. While the mem changes with the number of channels, the llc bw should be the same.
  %  \item we could propose a math foormula describing the Memory bandiwth throttling though the number of channels and LLC bandiwdth (supoosing that MBA splits perfectly the LLC BW)
%\end{itemize}

%The fig.~\ref{fig:min_lat_no_l2WB} and fig.~\ref{fig:min_lat_with_l2WB} show how the minimum memory fetching latency changes during the two different traffic conditions when a particular MBA delay is applied. \newline
%\begin{figure}
%\centering
%\includegraphics[width=.5\textwidth]{pictures/onecore_opcond0_thrott_var_512KB}\
%\caption{Minimum memory fetching latency without L2 WB\label{fig:min_lat_no_l2WB}}
%\end{figure}
%\begin{figure}
%\centering
%\includegraphics[width=.5\textwidth]{pictures/onecore_opcond1_thrott_var_512KB} \
%\caption{Minimum memory fetching latency with L2 WB\label{fig:min_lat_with_l2WB}}
%\end{figure}


%The MBA should act delaying requests going to the network of interconnect regardless of the other cores' behavior. So, by analyzing the throttling without contention, we can design properly the multicore analysis identifying the worst case condition. \newline




\subsection{The maximum available bandwidth}
We are interested in the minimum execution latency to quantify the maximum available bandwidth for an interference core.
We calculate in tab.~\ref{sec:fineg_max_throug_1op} the maximum number of memory reads in $T$ for each traffic condition $tr$ and MBA delay $d$:
\[
max(BW_{d}^{tr})=\frac{T*reqs_{read}}{min(L_{d}^{tr})};  \ T=min(L_{0}^{I}) 
\]
\[reqs_{read}=max(BW_{0}^{I})=8192
\]
Time window $T$ is the minimum execution latency for a core to fetch its 8192 cache lines when the MBA is disabled. \newline
Analyzing the percentages, we observe that 
\begin{itemize}
    \item the bandwidth in the 2nd operational condition for the delays 70, 80, and 90 is halved than the 1st operational condition.
    \item the other delays have no significant impact on the bandwidth limitation.
\end{itemize}
Why does Intel calibrate delays this way? Below, we justify these observations.
\subsubsection{70,80 and 90 delays}
Intel accounts memory write in the available bandwidth solving the write-back problem in the most straightforward and least architecturally expensive way. If our workload includes writing requests also, while the 1st operational condition does not change, the 2nd operational condition has a new worst case. The new worst case for the 2nd operating condition is when both memory read and memory write operations are required for each memory write request. Delaying L2 write-backs, potential memory writes (LLC write-backs) also are delayed\footnote{Note memory writing can be attributed to a particular physical core only if that physical core has its own LLC spatial partition}. Hence, we believe Intel also delays L2 write-backs in the 2nd operational condition preventing potential LLC write-backs. \newline
In conclusion, to prove our intuition, we reproduce in tab.~\ref{tab:onecore_finallatencies_WriteWorkload} and tab.~\ref{tab:onecore_finallatencies_WriteWorkload} the worst case for a memory write workload where each L2 write-back corresponds to one LLC write-back ($L2WBs=CASWrites$) in the 2nd operational condition. 
Note that:
\begin{enumerate}
    \item $max(BW_{R;d}^{I})=max(BW_{W;d}^{I})$ In the 1st operational condition, only memory reads are possible even if our workload includes memory write requests\footnote{memory write request (i.e., Read For Ownership RFO) consists in reading the cache line and updating the value in cache}. 
    \item $max(BW_{R;70:90}^{I})=max(BW_{W;70:90}^{II})$ The memory requests in the 1st or the 2nd operational condition. While in the 1st operational condition, we have only memory reads, in the 2nd, half of them are memory writes.
    \item $max(BW_{R;70:90}^{II})= \frac{max(BW_{W;70:90}^{II})}{2}$ The memory read requests in the 2nd operational condition for 70,80 and 90 delays are halved to prevent memory writes. This regulation choice is pessimistic because L2 write-back does not always cause LLC write-back and therefore writes to memory.
\end{enumerate}
In the multicore analysis, we choose to cover the correctness for the delays where the worst case of memory reads workload also includes the worst case for a memory write workload.
\subsubsection{Insignificant delays} remind that the MBA introduces an indirect memory bandwidth regulation. The delays are significant from requests going to the last level cache. Only a subset of them is also significant for the memory bandwidth. Probably, longer delays could impact too much on the LLC bandwidth regulation. 
\subsection{MBA variability}
MBA has low variability. The latency variability in tab.\ref{tab:onecore_finallatencies} is the same when there isn't throttling and when the MBA is enabled. The range of variability is around two thousand cycles. \newline 
Hence, the MBA is not a new source of variability, increasing its component reliability for a safety-critical context. Several sources explain this variability; however, the main factors are: 
\begin{itemize}
    \item DRAM refresh cycles are periodical. Two measurements can vary at most of two refresh cycles (around 1400 cpu cycles)
    \item Measures accuracy. The serialization instruction overhead is evaluated in our experiments (subsec.~\ref{measuremnt_tool}) with an error margin (around 200 cpu cycles)
\end{itemize}
The precision of MBA delays is surprisly, purticularly for the absence of outliers.
\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles for 8192 memory reads \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R;d}^{I})$ &144216 &144010 & 144494 & 144410\\[1pt]
$max(L_{R;d}^{I})$  &146010 & 146190 & 146468 & 146174
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &147532&147764&147556&149172\\[1pt]
$max(L_{R;d}^{II})$ &149510&149628&149754&150948
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R;d}^{I})$ &144294 & 146058 & 194466 & 287364\\[1pt]
$max(L_{R;d}^{I})$ &146010 & 147568 & 195470 & 288404
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &163376&282352&383132&566966\\[1pt]
$max(L_{R;d}^{II})$ &164708&283406&384116&567730
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{The maximum rate corresponding to minimum latency (memory read requests in $T$). \label{sec:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & & &  & \\
$max(BW_{R;d}^{I})$ &8192 &8192 & 8192 & 8192\\[1pt]
$max(BW_{R;d}^{I})\%$  &100\% &100\% & 100\% & 100\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R;d}^{II})$ &8024&8024&8024&7917\\[1pt]
$max(BW_{R;d}^{II})\%$ &98\%&98\%&98\%&97\%
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{R;d}^{I})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{R;d}^{I})\%$ &100\% &98\%  &74\%  &50\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R;d}^{II})$ &7237&4183&3080&2084\\[1pt]
$max(BW_{R;d}^{II})\%$ &88\%&51\%&38\%&25\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles for 8192 memory Read and 8192 memory write\label{tab:onecore_finallatencies_WriteWorkload}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{W;d}^{II})$ &198210&200704&196132&198230
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{W;d}^{II})$ &197715&283966&384918&565952
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{The maximum rate corresponding to minimum latency (read/write memory requests in $T$). \label{sec:fineg_max_throug_1op_write_workload}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & & &  & \\
$max(BW_{W;d}^{I})$ &8192 &8192 & 8192 & 8192\\[1pt]
$max(BW_{W;d}^{I})\%$  &64\% &64\% & 64\% & 64\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W;d}^{II})$ &2x6376&2x6376&2x6376&2x6376\\[1pt]
$max(BW_{W;d}^{II})\%$ &100\%&100\%&100\%&100\%
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{W;d}^{I})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{W;d}^{I})\%$ &64\% &63\%  &48\%  &33\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W;d}^{II})$ &2x6376&2x4183&2x3091&2x2097\\[1pt]
$max(BW_{W;d}^{II})\%$ &100\%&65\%&49\%&33\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}


























The multicore analysis quantifies the assured bandwidth when the MBA throttles the other cores. \newline
By the one core analysis, we identified two MBA operating conditions respectively when L2 WBs are present or not. This classification helps us to identify the worst case scenario with respect of the particular workload in input when the MBA throttles the interference cores. \newline
The memory load requests in the second operational condition are halved preventing LLC WBs. Hence, whenever in input there is a memory load workload, the worst case is reproduced by executing the interference cores in the first operational condition. \newline Contrarily, when in input there is a full-operational memory write workload, in the second operational condition, an interference core can achieve more bandwidth using the write-back flow. In conclusion, 
\begin{enumerate}
    \item for a memory load workload, an interference core has to be in the first operational condition (no L2WBs)
    \item for a full-operational memory write workload (where each L2WBs corresponds to LLC WBs), the worst case scenario is in the second operational condition including also the worst case for a memory load workload.
\end{enumerate}
Below, we show the worst case scenario for a memory load workload within a quad-core system. The three interference cores perform memory loads in the first operational condition and they are throttled with significant MBA-delays.
In the experiments, all four cores start with empty private caches. In this way:
\begin{enumerate}
\item the interference cores work in the first operating condition of the MBA (no L2 WB)
\item while the critical core emulates a critical task that fills its private caches.
\end{enumerate}
Workload details are listed in tab.~\ref{tab:manalyis_workload_details} 
\begin{table}
\caption{Workload details \label{tab:manalyis_workload_details}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
Scope & Initial state  &Memory fetching &Memory loads 
\tabularnewline
\hline 
\hline 
crit. task & L2 empty & 512KB  & 8192 
\tabularnewline
\hline 
interf. task & L2 empty & 768 KB & 12288

\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}
The tab.~\ref{tab:multicore_combinations_observed} shows how the maximum critical workload latency varies when the MBA throttles the cores with 80 and 90 delays. We sort the combinations in ascending order concerning the maximum latency of the critical task. \newline
For each experiment, we captured two hundred observations. \newline
We filter the data considering the number of load operations performed by the critical task (must be 8192) and a multicore synchronization validity test to capture the interference. 
%The maximum latencies respect the interference degree precedence.
\begin{table}
\caption{Critical core latency variability when the three interference cores are throttled by 70, 80 and 90 delay\label{tab:multicore_combinations_observed}}
\begin{center}
\begin{tabular}{  |c| c| c| c| }
\hline 
\#80 delay & \#90 delay & max latency (cpu cycles) 
\tabularnewline
\hline 
\hline 
0&3 & 243208 
\tabularnewline
\hline
1&2 & 260866 
\tabularnewline
\hline
2&1 & 299914 
\tabularnewline
\hline
3&0 & 313040  
\tabularnewline
\hline

\end{tabular}
\end{center}
\end{table}
%\textbf{Other possible experiments - multicore analysis:}
%\begin{itemize}
 %   \item increase the number of interference cores.
 %   \item try as workload interference a memory write workload testing all delays.
%\end{itemize}













\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles  \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R;d}^{I})$ &144216 &144010 & 144494 & 144410\\[1pt]
$max(L_{R;d}^{I})$  &146010 & 146190 & 146468 & 146174
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &147532&147764&147556&149172\\[1pt]
$max(L_{R;d}^{II})$ &149510&149628&149754&150948
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{W;d}^{II})$ &198210&200704&196132&198230
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R;d}^{I})$ &144294 & 146058 & 194466 & 287364\\[1pt]
$max(L_{R;d}^{I})$ &146010 & 147568 & 195470 & 288404
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &163376&282352&383132&566966\\[1pt]
$max(L_{R;d}^{II})$ &164708&283406&384116&567730
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{W;d}^{II})$ &197715&283966&384918&565952
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}






\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles  \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R;d}^{I})$ &144216 &144010 & 144494 & 144410\\[1pt]
$max(L_{R;d}^{I})$  &146010 & 146190 & 146468 & 146174\\[1pt]
$mean(L_{R;d}^{I})$ & 145331 &145306 & 145368 & 145368\\[1pt]
$CI(L_{R;d}^{I})_{99\%}$  & $\pm$181 & $\pm$165 & $\pm$180 & $\pm$154\\[1pt]
$accuracy(L_{R;d}^{I})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &147532&147764&147556&149172\\[1pt]
$max(L_{R;d}^{II})$ &149510&149628&149754&150948\\[1pt]
$mean(L_{R;d}^{II})$ & 148308 &148374 & 148387 & 150071\\[1pt]
$CI(L_{R;d}^{II})_{99\%}$  &$\pm$177 & $\pm$146 & $\pm$223 & $\pm$170\\[1pt]
$accuracy(L_{R;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &187598&185714&187664&187738\\[1pt]
$max(L_{W;d}^{II})$ &198210&200704&196132&198230\\[1pt]
$mean(L_{W;d}^{II})$ & 192111 &192802 & 192780 & 193377\\[1pt]
$CI(L_{W;d}^{II})_{99\%}$  &$\pm$931 & $\pm$1020 & $\pm$952 & $\pm$986\\[1pt]
$accuracy(L_{W;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R;d}^{I})$ &144294 & 146058 & 194466 & 287364\\[1pt]
$max(L_{R;d}^{I})$ &146010 & 147568 & 195470 & 288404\\[1pt]
$mean(L_{R;d}^{I})$ & 145316 &146760 & 195137 & 287735\\[1pt]
$CI(L_{R;d}^{I})_{99\%}$  &$\pm$154 & $\pm$128 & $\pm$92 & $\pm$89\\[1pt]
$accuracy(L_{R;d}^{I})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R;d}^{II})$ &163376&282352&383132&566966\\[1pt]
$max(L_{R;d}^{II})$ &164708&283406&384116&567730\\[1pt]
$mean(L_{R;d}^{II})$ & 164155 &282745 & 383543 & 567155\\[1pt]
$CI(L_{R;d}^{II})_{99\%}$  &$\pm$127 & $\pm$120 & $\pm$116 & $\pm$71\\[1pt]
$accuracy(L_{R;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W;d}^{II})$ &189228&281954&381588&562524\\[1pt]
$max(L_{W;d}^{II})$ &197715&283966&384918&565952\\[1pt]
$mean(L_{W;d}^{II})$ & 195011 &282832 & 382700 & 563612\\[1pt]
$CI(L_{W;d}^{II})_{99\%}$  &$\pm$698 & $\pm$188 & $\pm$274 & $\pm$330\\[1pt]
$accuracy(L_{W;d}^{II})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}






%Workload details are listed in tab.~\ref{tab:manalyis_workload_details}.\newline
{\color{blue}{The tab.~\ref{tab:multicore_combinations_observed} shows how the 99-percentile maximum critical workload latency varies when the MBA limits the interference cores with 80 and 90 delays (i.e., in the first row the three cores are limited with 90-delay). Note that we are assuming that the interference does not depend on the core position (i.e., if we limit the core 1 or the core 2 is indifferent).
We sort the combinations in ascending order concerning the maximum latency.}} 
For each experiment, we captured two hundred observations. \newline

%We filter the data considering the number of load operations performed by the critical task (must be 8192) and a multicore synchronization validity test to capture the interference. 

%\begin{table}
%\caption{Workload details \label{tab:manalyis_workload_details}}
%\begin{center}
%\begin{tabular}{ |c| c| c| c| c| }
%\hline 
%Scope & Initial state  &Memory fetching &Memory loads 
%\tabularnewline
%\hline 
%\hline 
%crit. task & L2 empty & 512KB  & 8192 
%\tabularnewline
%\hline 
%interf. task & L2 empty & 768 KB & 12288
%\tabularnewline
%\hline
%\end{tabular}
%\end{center}
%\end{table}


\begin{table}
\caption{Maximum critical latency when the three interference cores are throttled by 80 and 90 delay\label{tab:multicore_combinations_observed}}
\begin{center}
\begin{tabular}{  |c| c| c| c| }
\hline 
\#80 delay & \#90 delay & max latency (cpu cycles) 
\tabularnewline
\hline 
\hline 
0&3 & 243208 
\tabularnewline
\hline
1&2 & 260866 
\tabularnewline
\hline
2&1 & 299914 
\tabularnewline
\hline
3&0 & 313040  
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}






\begin{table}
\caption{Critical core latency variability when the three interference cores are throttled by 80 or 90 delay\label{tab:multicore_combinations_predicted}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline 
\#70d & \#80d & \#90d & $id$ calculation & resulting $id$ 
\tabularnewline
\hline 
\hline 
0&0&3 & $(0*(3/4)+3*(1/2)$ & $(1.5)id$
\tabularnewline
\hline
0&1&2 & $(1*(3/4)+2*(1/2)$ & $(1.75)id$
\tabularnewline
\hline
0&2&1 & $(2*(3/4)+1*(1/2)$ & $(2)id$
\tabularnewline
\hline
1&0&2 & $(1*(1)+0*(3/4)+2*(1/2)$ & $(2)id$
\tabularnewline
\hline
0&3&0 & $3*(3/4)+(0*(1/2)$ & $(2.25)id$ 
\tabularnewline
\hline
1&1&1 & $(1*(1)+1*(3/4)+1*(1/2)$ & $(2.25)id$
\tabularnewline
\hline
1&2&0 & $(1*(1)+2*(3/4)+0*(1/2)$ & $(2.5)id$
\tabularnewline
\hline
2&0&1 & $(2*(1)+0*(3/4)+1*(1/2)$ & $(2.5)id$
\tabularnewline
\hline
2&1&0 & $(2*(1)+0*(3/4)+1*(1/2)$ & $(2.75)id$
\tabularnewline
\hline
3&0&0 & $(3*(1)+0*(3/4)+0*(1/2)$ & $(3)id$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


==> old/copy_singlecore.tex <==
This section describes the single-core analysis results where the main goal was to estimate the indirect limitation of memory bandwidth when the MBA is enabled.
Below, we represent our results for the three workloads $R^{I}, R^{II}, W^{II}$. 
%Our experiments reproduce the first and the second operational condition in this way:
%our workload reads 2048KB in four granes of 512KB where the 1st and 2nd operational conditions are the first and third grane, respectively.
%he first grane is after the dynamic memory flush finding free space in cache, while the third grane is after reading 1MB, probably finding the private cache full being the L2 size of 1 MB. \newline
%Even though we achieve high precision in our measurements,
%the data are filtered like this (validity test):
%\begin{itemize}
%\item the number of last level cache misses must be equal to the number of memory reads ($ LLCmiss = CASreads = 8192$)
%\item in the 1st operational condition, the total L2 write-backs must be equal to zero ($L2WB = 0$)
%\item in the 2nd operational condition, the total L2 write-backs must be equal to the total memory requests ($L2WB = 8192$)
%\end {itemize}
%The numerical values are listed in tab.~\ref{tab:onecore_finallatencies} where the minimum and maximum workload latencies are associated with the respective environmental conditions. 
\subsection{Results representation}
The statistics out of 45 observations are listed in Tab.~\ref{tab:onecore_finallatencies} where 99\% mean confidence intervals are associated with the respective factors giving a degree of confidence of our measures. The accuracy also is always higher than 99\%.  %The mean latency represents well the latency distribution. We observed that the sample mode, mean and median fall in the same range of 100 cycles.
In addition, fig.~\ref{fig:boxplot_lat_onecoreanalysis} shows the boxplots for each experiment and a mean interpolation for the observations of the same workload and different MBA delays.
$L_{k;d}$ is the latency to execute the workload $k$ when the $d$ MBA delay is active. \newline
We are interested in the minimum execution latency to quantify the maximum available bandwidth for an interference core. We estimate this parameter through the observed minimum latency.
We calculate the maximum number of memory operations in $T$ as
\[
max(BW_{k;d})=\frac{T*max(BW_{R^{I};0})}{min(L_{k;d})}; 
\]
where time window $T$  is the minimum execution latency $min(L_{R^{I};0})$ for a core to fetch its 8192 ($max(BW_{R^{I};0})=8192$) cache lines when the MBA is disabled (0-delay). \newline
Tab.~\ref{sec:fineg_max_throug_1op} presents the maximum number of memory accesses in T only for the delays that have an important impact on the relative 0-delay observing the fig.~\ref{fig:boxplot_lat_onecoreanalysis}. In addition, we report also the percentage of synchronous bandwidth as
\[ max(BW_{k;d})\%= \frac{max(BW_{k;d})*100}{max(BW_{R^{I};0})} \]
Note that the synchronous memory bandwidth could be lower than the achievable memory bandwidth where also the memory writes are accounted (i.e., the workload $W^{II}$ achieves $150\%$ of synchronous bandwidth without a significant limitation). In Tab.~\ref{sec:fineg_max_throug_1op}, "2x" indicates double accesses regarding the memory writes.
\subsection{Results interpretation}
Observing the results, we note that:
\begin{enumerate}
    \item $max(BW_{R^{I};d})>max(BW_{R^{II};d})$ the less restrictive limitation for a memory read workload is when there aren't L2 write-backs.
    \item $max(BW_{R^{I};70:90})\approx max(BW_{W^{II};70:90})$ The maximum memory accesses in the 1st and in the 2nd operational condition is approximately the same for 70, 80 and 90 delays.
    \item $max(BW_{R^{II};70:90})\approx \frac{max(BW_{W^{II};70:90})}{2}$ The memory read requests in the 2nd operational condition for 70,80 and 90 delays are halved to prevent memory writes. This regulation choice is pessimistic because L2 write-back does not always cause LLC write-back and therefore writes to memory.
\end{enumerate}
{\color{red}{
The first observation give us an important alert for the future systematic MBA evaluation. When we test the memory bandwidth limitation for read operations, we have to focus our experiments on the first operational condition when there aren't L2 write-backs capturing the most permissive limitation. For instance, if we measure the limitation in terms of memory read requests in one millisecond probably we are considering the second operational condition and we are mistaking!}} \newline
{\color{magenta}{We discovered that even though some delays do not contribute on the indirect memory bandwidth limitation, the delays 70, 80 and 90 have an interesting behaviour. Indeed, they limit and conserve their limitation even if there are memory writes. In particularly, the 80 and 90 delays limit the memory synchronous bandwidth to 75\% and 50\% respectively, while the 70 delay avoids the overload of asynchronous requests halving the synchronous bandwidth in the second operational condition.}} \newline
For these reasons, in the multicore analysis, we choose to evaluate the assured bandwidth when the MBA limits the interference core only with 80 and 90 delays.
%For the insignificant delays remind that the MBA introduces an indirect memory bandwidth regulation. The delays are significant from requests going to the last level cache. Only a subset of them is also significant for the memory bandwidth. Probably, longer delays could impact too much on the LLC bandwidth regulation. 
\subsection{MBA variability}
MBA has low variability. The latency variability as difference between maximum and minimum latency, in tab.\ref{tab:onecore_finallatencies}, is the same (or lower) when there isn't throttling and when the MBA is enabled. Hence, the MBA is not a new source of variability, increasing its component reliability for a safety-critical context.  We tried also other workload size and the range of variability continuous to be around the same. 
The range of variability is around two thousand cycles for a read workload. Several sources explain this variability; however, the main factor are the peridoic DRAM refresh cycles. Two measurements can vary at most of two refresh cycles (around 1400 cpu cycles). The write workload, in addition, has the undisclosed hash function that maps the physical addresses to LLC slices. The structure in slice increases the access variability. \newline
The precision of MBA delays is surprisly, purticularly for the absence of outliers.





\renewcommand{\arraystretch}{1.5}
\begin{table}
\caption{Latency variability in terms of cpu cycles  \label{tab:onecore_finallatencies}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 00-delay  &10-delay &40-delay &50-delay 
\tabularnewline[1pt]
\hline 
\hline
%no L2 WB & & &  & \\
$min(L_{R^{I};d})$ &144216 &144010 & 144494 & 144410\\[1pt]
%$max(L_{R^{I};d})$  &146010 & 146190 & 146468 & 146174\\[1pt]
$mean(L_{R^{I};d})$ & 145331 &145306 & 145368 & 145368\\[1pt]
$CI(L_{R^{I};d})_{99\%}$  & $\pm$181 & $\pm$165 & $\pm$180 & $\pm$154
%$accuracy(L_{R^{I};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R^{II};d})$ &147532&147764&147556&149172\\[1pt]
%$max(L_{R^{II};d})$ &149510&149628&149754&150948\\[1pt]
$mean(L_{R^{II};d})$ & 148308 &148374 & 148387 & 150071\\[1pt]
$CI(L_{R^{II};d})_{99\%}$  &$\pm$177 & $\pm$146 & $\pm$223 & $\pm$170
%$accuracy(L_{R^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W^{II};d})$ &187598&185714&187664&187738\\[1pt]
%$max(L_{W^{II};d})$ &198210&200704&196132&198230\\[1pt]
$mean(L_{W^{II};d})$ & 192111 &192802 & 192780 & 193377\\[1pt]
$CI(L_{W^{II};d})_{99\%}$  &$\pm$931 & $\pm$1020 & $\pm$952 & $\pm$986
%$accuracy(L_{W^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
\hline 
\hline 
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$min(L_{R^{I};d})$ &144294 & 146058 & 194466 & 287364\\[1pt]
%$max(L_{R^{I};d})$ &146010 & 147568 & 195470 & 288404\\[1pt]
$mean(L_{R^{I};d})$ & 145316 &146760 & 195137 & 287735\\[1pt]
$CI(L_{R^{I};d})_{99\%}$  &$\pm$154 & $\pm$128 & $\pm$92 & $\pm$89
%$accuracy(L_{R^{I};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{R^{II};d})$ &163376&282352&383132&566966\\[1pt]
%$max(L_{R^{II};d})$ &164708&283406&384116&567730\\[1pt]
$mean(L_{R^{II};d})$ & 164155 &282745 & 383543 & 567155\\[1pt]
$CI(L_{R^{II};d})_{99\%}$  &$\pm$127 & $\pm$120 & $\pm$116 & $\pm$71
%$accuracy(L_{R^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$min(L_{W^{II};d})$ &189228&281954&381588&562524\\[1pt]
%$max(L_{W^{II};d})$ &197715&283966&384918&565952\\[1pt]
$mean(L_{W^{II};d})$ & 195011 &282832 & 382700 & 563612\\[1pt]
$CI(L_{W^{II};d})_{99\%}$  &$\pm$698 & $\pm$188 & $\pm$274 & $\pm$330
%$accuracy(L_{W^{II};d})$ &0.99 & 0.99 & 0.99 & 0.99
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{The maximum rate and the percentage of synchronous memory bandwidth corresponding to minimum latency (memory operations in $T$). \label{sec:fineg_max_throug_1op}}
\begin{center}
\begin{tabular}{ |c| c| c| c| c| }
\hline
Metric & 60-delay&70-delay &80-delay & 90-delay 
\tabularnewline[1pt]
\hline 
\hline 
%no L2 WB & &  &  & \\
$max(BW_{R^{I};d})$ &8192 & 8079 & 6080 & 4105\\[1pt]
$max(BW_{R^{I};d})\%$ &100\% &98\%  &74\%  &50\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{R^{II};d})$ &7237&4183&3080&2084\\[1pt]
$max(BW_{R^{II};d})\%$ &88\%&51\%&38\%&25\%
\tabularnewline[1pt]
\hline 
%with L2 WB &&&&\\
$max(BW_{W^{II};d})$ &2x6376&2x4183&2x3091&2x2097\\[1pt]
$max(BW_{W^{II};d})\%$ &155\%&101\%&75\%&51\%
\tabularnewline[1pt]
\hline
\end{tabular}
\end{center}
\end{table}
\begin{figure} 	
	\centering
	\includegraphics[width=0.47\textwidth]{pictures/boxplotAlldelaysCols.png}
	\caption{Boxplot latencies for the different workload and interpolation of the respective mean latencies  \label{fig:boxplot_lat_onecoreanalysis}}
\end{figure}









==> old/doe.tex <==
\textbf{\todo[inline]{Temporary UNLOCK: TUKL}}
\todo[inline]{GF: we should provide data on the statistical quality of the data, eg, confidence intervals (DONE We put the boxplots avoiding the huge table)}
\todo[inline]{GG: at some point we should mention exactly which processor (name) we used}
Our experiments are composed of two main analysis.
Single core analysis is a systematic approach to deriving the indirect memory bandwidth limitation achieved when the MBA delays the requests. 
Contrarily, the multicore analysis is focused on the guarantees rather than the limitation.
Multicore analysis tests the memory bandwidth achieved by a core executing a critical VM when the MBA (indirectly) limits memory accesses from 3 interfering cores (executing best-effort tasks).
Both, Single-core and multicore analysis, share the following architectural parameters (tab.~\ref{tab:share_parameters}).We use only one socket (one processor) composed of eight cores at most. We set the number of active cores via BIOS configuration. We only used one memory channel in both the analysis. 
%One DRAM channel throughput seems satisfying the core arrival rate. 
%In this architecture, six channels are plugable at most. 
In the BIOS, we set the DRAM refresh rate to periodic and the CPU core frequency to maximum (no power saving). These parameters helped to keep the latency variability to a minimum and maximize the memory requests rate. Similarly, we disabled the Pre-fetcher and Hyperthreading to reduce variability.
Next subsections present the design of experiments for both the analysis.
\begin{table}
\caption{Design of experiments: shared parameters \label{tab:share_parameters}}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
Shared parameters & setting
\tabularnewline
\hline 
\hline 
Socket & 1
\tabularnewline
\hline 
Used DRAM channel & 1
\tabularnewline
\hline 
Prefetcher & disabled 
\tabularnewline
\hline 
SMT &disabled
\tabularnewline
\hline
DRAM refresh cycles & periodic
\tabularnewline
\hline
core frequency &Maximum
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}


\subsection{Single-core analysis}
Single-core analysis has to estimate the maximum limitation for an interfering core when MBA is enabled with different delays (As per the Intel errata \cite{IntelRefManXeonScal}, delay values of 20 and 30 are erroneous on our processor and produce the same result as delay value 10).
Our experiments measures the latency execution variability for different kind of workloads.
\subsubsection{Memory read workload}
A read request in the worst case corresponds to a memory read operation when there is a LLC miss. Since we consider this worst case in our workload, read request and memory read operation are interchangeable terms.
However, we identify two different L2 traffic patterns for this worst case as a result of the LLC exclusivity in the processor. \newline
Inclusive and exclusive LLC handle an LLC miss differently. While an inclusive approach holds the new cache line into LLC and L2 keeping the inclusivity  [fig.\ref{llc_handling} (b)], the exclusive one fetches the new cache line only in private cache [fig.\ref{llc_handling} (a)].\newline These distinct approaches entail a different sequence of cache operations when there is a memory read.
In an inclusive architecture, the L2 writeback occurs only when the L2 set is full and the evicted L2 cache line is not updated (dirty) with the LLC copy[fig.\ref{llc_handling} (d)]. 
Therefore, there aren't L2 writebacks when we run only read requests in an inclusive architecture. Contrarily, in the exlusive architecture, we have L2 writeback whenever we read new memory  and the L2 set is full [fig.\ref{llc_handling} (c)]. 
\todo[inline]{GG: do we need to explain all this about inclusive and exclusive architecture or is it enough to explain why exclusive architecture causes 2 different traffic patterns?}
\begin{figure} 	
	\centering
	\includegraphics[width=0.45\textwidth]{pictures/llcmiss_handling.png}
	\caption{LLC miss handling in an inclusive and exclusive architecture respectively when there is space in L2 (a) (b) and when the L2-set is full (c) (d). We suppose available LLC space. \label{llc_handling}}
\end{figure}
The new Xeon processor (and so our micro-architecture) has an exclusive LLC.
Hence, our experiments include the two L2 traffic patterns as a factor. \newline
We prove our intuition in fig.\ref{fig:fineg_l2_wb_00} and fig.\ref{fig:fineg_l2_wb_90} where we fetch 2 MB of dynamic memory in several blocks of 64 KB when the MBA is disabled (0-delay) and enabled with 90-delay. 
While the above plot represents the latency (cpu cycles) for each block, the graph below shows the respective L2-WBs for each fetched block. The number of L2 write-backs grows as the L2 cache fills its capacity (L2 size is 1 MB). While initially L2 capacity is available and so there aren't L2 write-backs, when the L2 becomes full, each memory read sure corresponds to one L2 write-back (so 64KB of memory fetching correspond 1024 L2 write-backs). \newline
Noting the figures, we have two main observations. Without throttling (0-delay), the memory load latency does not change significantly when the L2 write-backs are present (fig.\ref{fig:fineg_l2_wb_00}) because L2 write-backs never cause LLC write-backs for a memory load workload. However the latency changes when the MBA is enabled (fig.\ref{fig:fineg_l2_wb_90}) on the two traffic patterns. The MBA probably  delays the L2 write-back requests. This explanation is entirely plausible because the controller should introduce a delay towards all outgoing requests on the interconnection network, thus also including reads and writes versus the last level cache. \newline
The second observation motivates the choice of consider L2 traffic pattern as a factor. The $R^{I}$ and $R^{II}$ in tab.~\ref{tab:doe_onecoreanalysis} represent respectively the read workload in the first operational condition (without L2 WBs) and in the second operational condition (with L2WBs).
In particularly, the read workload is composed of 8192 read requests where each request is an LLC miss ($ readReqs = LLCmiss = CASreads = 8192$) and hence a memory read operation. In $R^{I}$, the total L2 write-backs must be equal to zero ($L2WB = 0$), while in $R^{II}$, the total L2 write-backs must be equal to the total memory requests ($L2WB = 8192$).
These equalities serve as a validation test.
\subsubsection{Memory write workload}
write requests for a miss cache line in a write-back policy are memory reads operations until a dirty LLC cache line is evicted causing a memory write. Hence, since our write workload reproduces the worst case, every our write request causes one memory read and one memory write operation. The worst case of write requests has only one possible L2 traffic pattern because an LLC write-back is effect of an L2 write-back.
The $W^{II}$ in tab.~\ref{tab:doe_onecoreanalysis} represents this kind of workload.
In particularly, the $W^{II}$ workload is composed of 8192 write requests where each request is cause of one memory read and one memory write ($ writeReqs = LLCmiss = CASreads = CASwrites = 8192$). For the write workload only the second operational condition is possible since an LLC write-back is a consequence of L2 write back.
Agian, these equalities serve as a validation test.
%In conclusion the one-core analysis consists to evaluate the memory fetching latency when the MBA delays and traffic patterns change.
\begin{figure}
\centering
\includegraphics[width=.48\textwidth]{pictures/fineg_mba_thrott_latency_continuous_64KB_memory_fetching_delay0} \
\caption{2048 KB memory fetching in several blocks of 64KB when the MBA is disabled (0-delay)\label{fig:fineg_l2_wb_00}}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=.48\textwidth]{pictures/fineg_mba_thrott_latency_continuous_64KB_memory_fetching_delay9} \
\caption{2048 KB memory fetching in several blocks of 64KB when the MBA 90-delay is enabled\label{fig:fineg_l2_wb_90}}
\end{figure}
\subsection{Multi-core analysis}
While the single-core analysis gives us information about the memory access limitation when the MBA-delay and workload are fixed, the multi-core analysis analyzes the assured bandwidth for a critical core when the MBA limits the other ones. 
In the multi-core analysis, we deploy a quad-core system evaluating how changes the assured bandwidth when there is interference.\newline
In particularly, we consider a specific case where one critical core fetches its dynamic memory without MBA throttling, while the other three cores create interference accessing the memory with maximum rate and they are limited by the MBA. \newline
The range of delays and the particular workload considered for the interference cores will depend on the result of single-core analysis focusing the analysis in the worst-case.In addition, we interpret the observed data thorough a model.
\subsection{Measurement tool and workload considerations \label{measuremnt_tool}}
We performed experiments in Linux as the high server boot duration (several minutes) makes it time consuming to do bare-metal development and experimentation. \newline
%In particularly, we decompose our memory load workload in several configurable blocks focusing our observation on different traffic patterns (Fig.~\ref{exec_model_exp}).
Our measurement tool captures the latency and several factors (such as LLC writeback, L2 writeback and CAS commands) of a particular workload. The latency is captured in terms of TSC (Timestamp counter). The fixed TSC frequency is close to the maximum CPU frequency, hence, we refer to TSC cycles as cpu cycles. We favor the latency rather than bandwidth measurements because the latter requires a regulation period limiting the resolution. \newline
%Below, we describe some considerations that we used for precise experiments in x86:
%\begin{itemize}
   % \item the workload and tool run in kernel space avoiding the context switch for the MSR (Model specific register) access and disabling kernel preemption
   % \item The latency is captured in terms of TSC (Timestamp counter). The fixed TSC frequency is close to the maximum CPU frequency. For these reason, we refer to TSC cycles as cpu cycles.
   % \item we use serialization instructions (as fence) to create independent phase and observation, and to keep the instruction order when necessary (i.e., for reading TSC). The overhead of these instructions have to be not considered in the measurements.
%\end{itemize}
%As shown in fig.~\ref{exec_model_exp}, the experiments are repeated overtime.
%Before the execution, each experiment reproduces memory operations flushing the dynamic memory and so cleaning the cache space. \newline
%In this way, we don't reproduce the memory operations as LLC capacity misses because, in our architecture, reading a dynamic memory bigger than entire cache space is not a sufficient condition to ensure a miss. This is due to the undisclosed hash function that binds physical address and LLC slice. \newline
%\begin{figure} 	
%	\centering
%	\includegraphics[width=0.45\textwidth]{pictures/Observation.png}
%	\caption{Experiment execution model \label{exec_model_exp}}
%\end{figure}
The interference workload is wrote in assembly and consists in only read or write operations (full-loop unrolling). The accessed addresses have a stride 
equals to the cache line size\footnote{Our cache line size is 64 Bytes}. The full loop unrolling of memory requests reproduces the maximum arrival rate and so the maximum interference. Even though the loop unrolling of memory requests increases the code size, we design our experiments controlling the absence of extra LLC misses. \newline
We reproduce the two L2 traffic patterns for a read workload through some initial setup operations. To avoid L2 write-backs and to have memory accesses, we flush the dynamic memory before the workload execution, while to reproduce L2 write-backs for the $R^{II}$ workload, we execute also a pre-read workload to fill the L2 cache. \newline
Contrarily, for the write workload $W^{II}$, we reproduce the worst case executing a pre-workload of write-requests filling the entire cache space of dirty and useless cache-lines. In addition to synchronous memory accesses, the dirty cache lines assure LLC write-back (memory write) whenever there is an LLC eviction.

\begin{table}
\caption{Design of experiments: single-core analysis \label{tab:doe_onecoreanalysis}}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
Goal & Quantify and evaluate the MBA \\ &throttling without memory interference
\tabularnewline
\hline 
\hline 
Parameters & setting
\tabularnewline
\hline 
 cores & 1 
\tabularnewline
\hline 
\hline 
Factors & Values
\tabularnewline
\hline 
MBA & delay $d$, $d\in \{10; 40; 50; 60; 70; 80; 90\}$
\tabularnewline
\hline
workload & \begin{tabular}{ c| c| c }
$R^{I}:$ \{&$R^{II}$: \{ &$W^{II}$: \{ \\8192 CAS R;&8192 CAS R;&8192 CAS R;
\\no L2WBs;&with L2WBs;&with L2WBs;
\\no LLCWBs\}&no LLCWBs\}&with LLCWBs\}
\end{tabular}
\tabularnewline
\hline 
\hline 
Metric & Description
\tabularnewline
\hline 
Latency & memory fetching latency in terms of cpu cycle\\&
\{$L_{R^{I};d}$;$L_{R^{II};d}$;$L_{W^{II};d}$\}
\tabularnewline
\hline
Obs. & $45$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{Design of experiments: multi core analysis}
\begin{center}
\begin{tabular}{ |c| c| }
\hline 
Goal & Quantify and explain \\& the critical core assured bandwidth \\& when the MBA limits the interference\\& cores with significant delays
\tabularnewline
\hline 
\hline 
\hline 
Parameters & setting
\tabularnewline
\hline 
 cores & 1 critical core and 3 interference cores
\tabularnewline
\hline 
int.workload & $k \ depends \ on \ the \ single \ core \ analysis$
\tabularnewline
\hline crit. workload & $R^{I}: \{8192 \ CAS \ R, no \ L2WBs, no \ LLCWBs\}$
\tabularnewline
\hline 
\hline 
Factors & Values
\tabularnewline
\hline 
MBA & delay $d_{i={1,2,3}}$ for the i-th interference core \\& $d_i\in \{10;40; 50; 60; 70; 80; 90\}$
\tabularnewline
\hline 
\hline 
Metric & Description
\tabularnewline
\hline 
Latency & critical memory fetching latency in terms of cpu cycle\\&
\{$L_{k;(d_1,d_2,d_3)}$\}
\tabularnewline
\hline 
Obs. & $45$
\tabularnewline
\hline
\end{tabular}
\end{center}
\end{table}




==> old/introduction.tex <==

\todo[inline]{lock Marcello}
%\textbf{@ALL} \textbf{Time-sensitive cloud motivations} \newline
%- leverage the cloud advantages as the workload elasticity, performance, maintainability, \newline
%- reliability - fault tolerance, critical task throttling the no critical task. \newline
%- maximizing the average resource utilization (power efficiency)

As seen in Ericson's Computing Fabric  \cite{ericsson}, and railway use case of EU projects such as SECREDAS \cite{gala:railway}, industries are exploring cloud computing for hosting safety-critical applications as clouds support ease of re-usability, maintainability, and reconfiguration while providing workload elasticity and higher availability. Thus, clouds help industries in reducing their running costs and carbon footprint. Moreover, industries can sell safety-critical operation as a cloud-based service.

Industries can execute existing safety-critical applications without any significant modifications as Virtual Machines (VMs) in a cloud computing environment. These safety-critical VMs run must alongside other non-critical/best-effort VMs executing in the cloud. All VMs are unaware that they are running in a virtualized environment or know the actual underlying cloud nodes or hardware resources.

Cloud nodes are composed of COTS multicore processors. Multicore architectures are rich in shared resources adding new forms of non-determinism for safety-critical applications. Even though current resource sharing approaches allow fast communication and improve the average resource utilization, shared resources introduce several dependencies (in space and time) between parallel flows complicating the analysis of the Worst-Case Execution Time (WCET). In particular, co-executing tasks or VMs add a new circular dependency between the scheduling and WCET analysis; the scheduling uses the WCET to decide on a schedule, while the WCET analysis itself depends on the schedule of the other cores of the same node. \newline

This results in clouds being non-deterministic as they do not provide resource allocation guarantees to the VMs.
Contrarily, safety-critical VMs depend on the guaranteed and timely allocation of resources to ensure their end-to-end deadlines are met. 
These uncertainties of current cloud models impedes their adoption in safety-critical domains.

Several existing safety standards adopt the concept of strict spatial and temporal partitioning, such as ARINC 653 specification.
Partitioning reduces analysis complexity and opens the previous circular dependency enabling incremental development and certification (iD\&C) paradigm \cite{4702768}. \newline
Mainly, we can use a three-dimensional space to identify the where contention occurs, and thus, the resolution for that cause of contention:
\begin{itemize}
    \item flows in conflict: what kind of flows are in conflict. Conflicting instructions can be of the same task (in a VM) or of two different tasks (potentially from two different VMs);
    \item kind of contention: what source is contended. Mainly, the sources of contention are the resource storage and resource throughput. 
    \item context: where is the conflict. Principally, shared resources are within a physical intra-core or inter-core context.
\end{itemize}

In this paper, we are interested on the temporal contention, in particularly for the memory (controller) accesses from co-executing tasks/VMs allocated to different hardware cores. Memory access contention has special attention for two main reasons:
\begin{itemize}
    \item Memory accesses are unavoidable.
    \item Considering the worst case memory access latency (the maximum contention) for the memory accesses can increase the WCET by several orders in magnitude, particularly with increase in number of co-accessing cores \cite{Nowotsch2013, Pellizzoni2010WorstCD}.
\end{itemize}

Therefore, below, we introduce the temporal contention starting from intra-core context moving versus our interest inter-core context. Even if spatial contention is not our main topic, we describe how it is coupled with memory temporal contention.
Inside a private core context, instructions (ILP) and multiple hardware threads, as a result of simultaneous multi-threading (SMT), contend simultaneously for access to several resources such as functional units and caches, improving private resource utilization. The literature does not still address interference from SMT (e.g., Hyper-threading in Intel processors) as this feature can be easily disabled. \sout{Even if, this feature could be investigated for a deterministic temporal throttling role being a standard feature on modern cloud platforms.}\todo{GG: do we need this sentence; it is grammatically incorrect and I am not sure what you want to say here}
Contrarily, the contention of functional units between parallel instructions is a well-known source of temporal anomalies \cite{Lundqvist1999TimingAI}\cite{Reineke2006ADA}. It can be handled by several serialization instructions restoring the program order or by increasing the analysis complexity.
While the intra-core interference can be analyzed or avoided without impacting the overall system utilization, a non-efficient algorithm for inter-core interference affects the entire system performance. 
On the modern multicore system, several cores (or hardware threads) share several resources such as a last level cache (LLC), network of interconnect and memory.

\sout{Even though spatial contention is not our main topic,} The spatial contention in the LLC has a significant impact on the memory access contention as LLC writebacks lead to asynchronous memory accesses.
While synchronous memory accesses are "synchronous" only with the requester demand, these asynchronous memory accesses depend on the memory requests from cores as the LLC is shared.
This means that temporal memory access partitioning is not possible until we do not have LLC spatial partitioning.
The main software solution for LLC spatial partitioning is horizontal partitioning leveraging the MMU (Memory Mapping Unit). Even if this solution is configurable on almost any architectures, horizontal partitioning implicitly divides the memory space, and thus, reducing page choices. Hence, special hardware support for cache way-partitioning (vertical partitioning) is favorable, e.g., Intel's Cache Allocation Technology (CAT) \cite{IntelRefManXeonScal}.
While LLC partitioning allows to identify distinct core flows versus the memory\todo{GG: not clear what you want to say here}, how to regulate these flows continuous is an open question. 

Existing work propose several memory access regulation methods to limit the maximum interference for the worst case memory access latency analysis.
\sout{Nowadays, the most suitable approach for temporal partitioning is resource limitation.}
The basic idea is to limit the memory accesses from individual cores for each regulation period. Thus, it is possible to distribute the available memory access bandwidth and obtain a tighter worst case memory access latency bound.
Software-based resource limitation approaches, such as Memguard \cite{Yun2013MemGuardMB}, require monitoring the memory requests from each core and applying a throttling policy to prevent memory accesses from cores that have deleted the assigned memory budget for that regulation period.
Despite the simplicity of design of software-based approaches, it is not possible to achieve high resolution and efficiency as:
\begin{itemize}
    \item The high overhead of the approaches and the possible timer resolution limit the regulation period duration (coarse-grained regulation period) impacting the resolution
    \item The throttling policy of the approaches involve stopping the core execution for preventing memory access.  Such a throttling policy is not suitable for a cloud as a core cannot continue its execution within the private context, such as private caches and functional units, reducing the private resources utilization. \newline 
\end{itemize}

Hardware architectures support only the monitoring synchronous per-core memory accesses through a non-architectural performance monitoring event (independent of the architecture). Since existing approaches leverage performance monitoring counters (PMC), they monitor only synchronous memory requests and do not consider memory accesses from asynchronous write-backs.

Intel proposed a new hardware feature with know as Memory bandwidth allocation (MBA) in its new Xeon processors \cite{IntelRefManXeonScal}. 
The MBA delays the requests going to the interconnect from a core's private context. MBA provides configurable nine delay values between $10$ to $90$ in increments of $10$. We can use to apply indirect memory bandwidth throttling.
This controller overcomes the limitations of software base-approaches: (1) we have a fine-grained regulation period because the delays are inserted by hardware between requests (2) a hardware based based method does not require software intervention except for the initial setup (3) the core execution is not stopped to prevent memory access preserving the private resource utilization.

However, the name, Memory bandwidth allocation (MBA), is misleading. The MBA controller only introduces delays between the core private context and the shared context and does not directly allocate memory bandwidth to cores. The memory bandwidth allocation/regulation is an indirect consequence of the introduced delay. Hence, our evaluation contributes to derive the indirect memory bandwidth achieved by cores for providing real-time guarantees. 
%our main contribution regards the Intel MBA assessment as an indirect memory bandwidth regulation controller for real-time.
Mainly,
\begin{enumerate}
    \item {\color{red}{We propose a systematic approach to derive the indirect memory bandwidth limitation.}}
    \item {\color{magenta}{We experimentally prove that the 70, 80 and 90 MBA delay values limit the memory bandwidth even if there are LLC write-backs (asynchronous memory accesses), while the remaining MBA delay values are not significant.}}
    \item {\color{blue}{We test the assured bandwidth for a core allocated to a critical VM when the MBA limits the bandwidth of three interference cores with three significant MBA delay values.}}
    \item {\color{violet}{We propose a prediction model to interpret the assured bandwidth.}}
\end{enumerate}
\begin{figure} 	
	\centering
	\includegraphics[width=0.47\textwidth]{pictures/architecture.png}
	\caption{Abstract Intel Socket memory hierarchy with MBA  \label{fig:architecture}}
\end{figure}

%\begin{enumerate}
    %\item We describe how to derive the achievable memory bandwidth from a particular delay regarding different sources of variability for a memory load workload. In addition, we investigate the component reliability comparing the variability with and without MBA throttling.
   % \item afterward, we test the critical assured bandwidth in the identified worst-case traffic pattern when the MBA throttles the interference cores.
    %\item in conclusion, we interpret these critical memory bandwidth observations by a predicting model and we conclude our assessment comparing the target MBA with the state of art MemGuard.
%\end{enumerate}




==> old/new_Intel_capabilities.tex <==
\todo[inline]{temporary UNLOCK: TUKL}
The technological evolution of Intel server micro-architectures can be summarized by passing from the Broadwell to the Skylake-server architecture\footnote{Note our micro-architecture is a CascadeLake. The CascadeLake inherits the presented Skylake-server arichitectural characteristics.}. \newline
The socket of both is composed of several core private contexts and one shared context.
\begin{itemize}
\item Each private context encloses the core with its private caches (L1 and L2).
\item while all private contexts share and contend the network of interconnect, the last level cache, and the DRAM memory.
\end{itemize}
The main differences are the network of interconnect and the inclusiveness of the last level cache.
\begin{itemize}
\item The new Sky-lake server have a Mesh rather than a Ring. Mesh increases request throughput by scaling with the number of cores.
\todo[inline]{GG: do we need so much history about "technological evolution" of intel architecture or can we start directly from the relevant parts of the Skylake architecture? e.g. RDT and LLC. It seems that we are using quite a lot of space for giving information not directly relevant to the hardware under study}
\item The last level cache in the Skylake-server micro-architectures is not inclusive (exclusive). An LLC exclusive frees the last level cache to be as large as the sum of all core private caches. Since it doesn't need the LLC inclusiveness of all cache lines.  However, usually, it requires a bigger directory that holds (theoretically) the state of all cache lines. \newline 
The exclusive LLC fits the scalability needs of the modern micro-architecture complicating the coherency protocol. 
We can have multiple cores with their larger private cache without increasing LLC space. For example, we went from a 254KB L2 with Broadwell to a 1MB L2 with the SkyLake-server. \newline
The second advantage is the efficiency.
While the cache lines are replicated in the inclusive LLC, the exlusive model enables to keep different cache lines in LLC and in private caches.
\end{itemize}
The new Intel Xeon Scalable processors have a Cascade-Lake or Ice-Lake micro-architecture inheriting all the features presented for the Sckylake Server. \newline
Furthermore, these new Intel processors support temporal and spatial isolation at the hardware level through Resource Director Technology (RDT). We can associate spatial and temporal properties with class of service (CLOS) and then bind the CLOS to a virtual core. \newline
One core cannot change the class of service of another core. However, it can configure the properties of any CLOS. \newline
RDT makes available monitoring and allocation features.
\subsection{RDT monitoring features}
The RDT monitoring features of the RDT do not support interrupt mechanisms. The monitoring data must be read synchronously (polling). \newline
In addition to the service class, we can associate a RID (Resource ID) to each virtual core. \newline
Multiple cores with the same RID correspond from a monitoring perspective to a single resource (RID). \newline
We can monitor a two properties of a RID:
\begin{itemize}
\item the occupancy (in bytes) of the last level cache
\item the outgoing band from the LLC towards the memory (total bandwidth) and the outgoing one towards the local processor memory (internal bandwidth)
\end{itemize}

\subsection{RDT allocation features}
RDT allocation features enables the inter-core resource partitioning.
\subsubsection{CAT and CDP}
The Cache Allocation Technology (CAT) implements a cache way-partitioning at the hardware level of the Last Level Cache.
We can define the number of ways for a class of service (CLOS) through a bitmask (of contiguous bits). This mask can isolate the CLOS cache capacity and still control its overlapping with others. \newline
The CDP (Code and Data Prioritization) extends the functionality of the CAT by specializing it in Data and Code. \newline
With this functionality, a class of service can partition its cache capacity into Data and Code.
\subsubsection{MBA}
The Memory Bandwidth Allocation (MBA) allows to allocate the available physical core memory bandwidth. The MBA controls a configurable delay for requests going to the interconnect network from the core private context. By these delays, we can apply an indirect throttling policy in memory access without impacting the use of private resources. We can associate the MBA delay with a class of service. If two virtual cores of the same physical core have different delays, the larger delay will override the other.

==> old/related_work.tex <==
\sout{Memory latency is a well-known source of non-determinism in safety-critical (real-time) applications. Even though a task spends only 10 \% of its life cycle to fetch memory, the execution time can increase by 300 \% in an eight-core system due to worst-case memory interference \cite{Pellizzoni2010WorstCD}.} 
The maximum latency variability can be reduced through memory bank aware partitioning because the memory banks work in parallel.
PALLOC \cite{Yun2014PALLOCDB} enables mapping between the memory pages and the physical banks leveraging the MMU. We can change the bank allocation at run-time. \newline
However, few banks reduce the memory level parallelism (MLP), impacting the average performance. \newline
Even though bank partitioning reduces the latency variability, the temporal contention of upstream resources such as the network of interconnect and memory controller or shared banks remains unmanaged.\newline
Under a worst-case perspective, each access incurs the worst-case interference without a predictable analysis or regulation. Below, we extend the classification of \cite{Kotaba2013MulticoreIR} distinguishing analysis and regulation (partitioning) methods. \newline These two macro-classes respectively know or define the maximum processing element interference. 

\subsection{Analyze the interference \label{sec:anal_interf}}
The idea is to know the maximum number of conflicts through static analysis. Under a worst-case perspective, the first goal is to classify each access for what hierarchy memory level will address. Such analysis gets complicated with shared caches. In \cite{Liang2009TimingAO} each access is first analyzed in the absence of inter-core cache conflicts, and subsequently, a separate inter-core cache conflict analysis refines each classified access. \cite{Chattopadhyay2013ScalableAP} improves the estimation of inter-core cache conflicts combining abstract interpretation and path-sensitive verification (e.g., model checking and symbolic execution). In \cite{Chattopadhyay2010ModelingSC}, \cite{Kelter2011BusAwareMW}, \cite{Chattopadhyay2012AUW} shared cache and bus analysis are combined, applying a TDMA bus arbitration. \newline
Interesting is how \cite{Chattopadhyay2010ModelingSC} resolves the circular dependency between the bus and cache analysis. Indeed, conflicts on the shared resource occur when two tasks overlap over time. However, this requires knowing the lifetime of the tasks. By assuming a compositional architecture, \cite{Chattopadhyay2010ModelingSC} can define a valid initial state and resolve the circular dependency. \newline
These analysis approaches have the following drawbacks: 
\begin{itemize}
\item the computational complexity increases with the number of tasks under analysis.
\item the arbiter is supposed to be deterministic as TDMA. However, on the modern COTS there are more optimization policies
\item there are no independent partitions. The solution validity is straight coupled with tasks under analysis.
\end{itemize}
However, probably, this is the precise-way to achieve the tightest bound estimate. So we believe access classifications suitable within a partition where the tasks under analysis are limited or as hint for the partitioning. \newline

\subsection{Regulate the interference \label{sec:regulate_approaches}}
These approaches handle the interference regulating or serializing the accesses.
\subsubsection{Execution model}
The basic idea of execution models is to split the real-time task into different phases and then enforce a high-level co-scheduling mechanism. \newline
The co-scheduler rules implicitly define the contention degree without relying on low-level arbiters.
The accesses are serialized in several phases, and these phases can be overlapped by co-scheduler achieving a predictable degree of interference. \newline
In \cite{Pellizzoni2011APE}, \cite{Boniol2012DeterministicEM} the co-scheduler implements a TDMA policy. However, a TDMA policy is not scalable with the number of cores. \newline
Pellizzoni \cite{Pellizzoni2011APE} proposes PREM handling the contention of main memory between a single-core and several peripherals. While Boniol\cite{Boniol2012DeterministicEM} extends the concept of the execution model to a multicore platform dividing the execution phase into communication and local execution slices. \newline
The execution models require program or compiler modifications. Boniol \cite{Boniol2012DeterministicEM} also proposes a development process and an automated toolset for the designer to program a sliced architecture.

\subsubsection{Resource limitation}
These approaches make predictable and deterministic the maximum interference limiting the processing element accesses. \newline 
They regulate the interference without modifying or statically analyzing the program. \newline This solution needs a throttling policy to stop the processing element access and a monitoring policy for issued request counting. \newline
The first to perceive the potentiality of performance counters to monitor shared resource accesses has been Bellosa \cite{Bellosa1997ProcessCC}, \cite{Bellosa1999TheTD}. Notably, \cite{Bellosa1997ProcessCC} captures on each PE the only interesting available events such as last-level cache hits and references to extract the LLC misses. The LLC-misses represents the processing element synchronous accesses. \newline
Subsequently, the "LLC misses" are available as a non-architectural event on modern COTS. Yun \cite{Yun2012MemoryAC, Yun2013MemGuardMB} indeed leverages this event to monitor the PE accesses. \newline
As throttling policy, Bellosa \cite{Bellosa1997ProcessCC} inserts idle-loop inside TLB-miss handler, while Yun \cite{Yun2012MemoryAC, Yun2013MemGuardMB} deschedules the task from queue-running tasks.
Bellosa explicitly hints processor constructors to add a programmable delay between load/store operations \cite{Bellosa1997ProcessCC}. \sout{Maybe the Intel MBA is the result of this advice.} \newline
Resource limitation software approach share the following drawbacks:
\begin{itemize}
    \item efficiency: they prevent access to the shared resource forbidding the processing element execution reducing the overall system utilization.
    \item resolution: a software implementation limits the achievable resolution concerning handler sub-routine overhead and timer resolution in the regulation period.
\end{itemize}
%In summary, by limiting the number of PE accesses inside a regulation period, we can define a maximum predictable interference. This prevention algorithm can degrade average performance: the not-consumed PE bandwidth would be lost. 
%So Memguard \cite{Yun2013MemGuardMB}  tries to fill this efficiency gap by defining a reclaimable bandwidth into soft-realtime context. Furthermore, the processing elements are free to execute whenever the assured bandwidth is consumed within the regulation period. \newline
%The second observation is about the policy of throttling. \newline
%Resource limitation software solutions prevent access to the shared resource forbidding the processing element execution reducing the overall system utilization. Furthermore, a software implementation limits the achievable resolution concerning handler sub-routine overhead and timer resolution in the regulation period. \newline

\todo[inline]{GG: I think \cite{Nowotsch2013} is missing}.

==> rebuttal.tex <==

\section{Rebuttal ISORC 2022}
The ISORC 2022 rebuttal
period will be between 2022-03-22 and 2022-03-27.

During this time, you will have access to the current state of your
reviews and have the opportunity to submit a response of up to 500
words. Please keep in mind the following during this process:

* The response must focus on any factual errors in the reviews and
any questions posed by the reviewers. It must not provide new
research results or reformulate the presentation. Try to be as
concise and to the point as possible.

* The rebuttal period is an opportunity to react to the reviews, but
not a requirement to do so. Thus, if you feel the reviews are
accurate and the reviewers have not asked any questions, then you do
not have to respond.

* The reviews are as submitted by the PC members, without any
coordination between them. Thus, there may be inconsistencies.
Furthermore, these are not the final versions of the reviews. The
reviews can later be updated to take into account the discussions at
the program committee meeting, and we may find it necessary to
solicit other outside reviews after the rebuttal period.

* The program committee will read your responses carefully and take
this information into account during the discussions. On the other
hand, the program committee will not directly respond to your
responses, either before the program committee meeting or in the
final versions of the reviews.

* Your response will be seen by all PC members who have access to the
discussion of your paper, so please try to be polite and constructive.

The reviews on your paper are attached to this letter. To submit your
response you should log on the EasyChair Web page for ISORC 2022 and
select your submission on the menu.


\subsection{Review 1}
%----------- Overall evaluation -----------
SCORE: 0 (borderline paper) \newline
%----- TEXT:
The authors discuss the effectiveness of the memory bandwidth allocation (MBA) technology available in Xeon Processors with RDT (resource director technologies). They show that only a subset of settings are effective. Moreover, the authors explore the memory bandwidth that can be assured to a single core when other cores interfere with concurrent memory accesses.

The design of experiments proposed in the paper is solid. In the "single-core analysis" the memory bandwidth limitation capabilities of MBA are investigated, whereas in the "multi-core analysis" the capabilities of MBA to guarantee memory bandwidth are explored.

The experiments are very interesting and show the current "state of affairs" concerning the capabilities of MBA in controlling memory contention. 
\newline 
\textbf{Since RDT is still a moving target and differs from generation to generation of RDT compatible Xeon processors I am a little hesitant to recommend to accept the paper for a conference.} 


\newline
For me the results are rather suitable to be discussed in a workshop setting since they might very well be outdated in a few month. For that reason the paper is borderline for me. Even if it is well written and the experiments are extremely well conducted.

\subsection{Review 2}
%----------- Overall evaluation -----------
SCORE: 0 (borderline paper) \newline
%----- TEXT:
The authors analyse multicore processors in respect to bandwidth allocation limits due common memory accesses of different cores which may affect or harm each other. They specifically address Intel's memory bandwidth allocation (MBA) technology and perform different evaluations to demonstrate its abilities and limitations. They present the overall architecture of MBA as well as their evaluation settings and the evaluations.

I like the topic of the paper and think it fits in the scope of ISORC, but I think the paper should be structured more clearly and provide more details: \newline
\begin{itemize}
    \item \textbf{Page 3: "We can asociate spatial and temporal properties with a class of service (CLOS) and then bind the CLOS to a virtual core."
Which properties do you mean? What is the impact a CLOS has to the system?}
    \item In addition, please sketch what the Resource Directir Technology does.
    \item \textbf{You write that you disabled the pre-fetcher as well as Hyperthreading to reduce variability. This is highly abstract. I assume you mean varability with respect to bandwith allocation. Is that right?}
    yes, the hyperthreading can interfere in the access to the memory because the two virtual cores on the same physical core share the available pending requests versus the memory, and the hardware (and softare) pre-fetcher can bring in cache a predictable number of cache lines making the successive requests LLC hits rather than LLC miss.
    Such behavior makes hard to achieve the maximum arrival rates in the single core analysis, furthermore, the hardware pre-fetcher is shared between the cores making difficult also the multi-core analysis.
    \item Table I and II need to be explained. Please try to place them to the next page where the explanations can be found. 
    \item Page 4: Please state in detail the difference of the single-core and the multi-core analysis. From your description, also the single-core analysis takes several cores into account. 
    \item \textbf{Page 4. What do you mean by "The number of observations achieves more than 99\% of accuracy."? Please explain.} The accuracy is calculated as the mean confidence interval calculated with 99\% of confidence divided by the sample mean
    
    \item \textbf{Page 4: What do you mean by "exclusive" and "inclusive" architecture? }
    Inclusive LLC includes all the cache lines holding in private caches. After an LLC miss, in an inclusive LLC the new cache-line is brought both in LLC and private cache keeping the inclusiveness, while in an exclusive LLC the new cache line is brought only in private cache. Hence, being an L2 a private cache as we can see by fig.1, in an exclusive architecture we have an L2 WB whenever the set is full even though the evicted cache-line is clean. Contrarily, in an inclusive LLC, being a copy in LLC, if the new cache-line is clean, the L2 writeback is not necessary. 
    
    \item \textbf{Page 4: What is meant by the "latency (cpu cycles)" exactly? The number of processor cycles to fetch a 64 KB block?} yes, in fig.2 and fig.3 are the processor cycles to fetch 64 KB.
    \item \textbf{Page 4: I assume the delay is measured as percentage. Please define it exactly.}
    As we can see by the Tab. I and II, the MBA delay is configurable value between 10, 20, 30, 40, 50, 60, 70, 80, 90. In our architecture, we don't have the value 20, 30 (as explained in page 4, Single-core Analysis, 4 line, "Intel errata"). 
    \item \textbf{Page 5: "The multicore analysis requires thirty observations to achieve a 99\% accuracy." What does this mean?}
    The accuracy is calculated as the mean confidence interval calculated with 99\% of confidence divided by the sample mean. Thirty observations are sufficient to achieve a 99 \% of accuracy.
    \item \textbf{Page 5: "The number of 8192 requests (meaning 512KB of memory fetching) has been chosen since it assures us to not have L2WBs in RI". How does the 2\^13=8192 requests relate to 512KB of memory?} Each request is a cache line (64 byte) as explained in page 5, Measurement tool and workload considerations, "he workload as consecutive memory operations (full-loop unrolling) and choosing a stride between consecutive accesses equal to the cache line size (our cache line size is 64 Bytes)."
    \item \textbf{Please describe in details the differences and motivation for RI and RII and WII}
    
    \item Chapter V.B: Please introduce more structure: Tell the lessens you learned (e.g. in separate paragraphs) and explain them. 
    \item Page 7: Motivate the "interference degree" in details and provide an example. 

\end{itemize}





\subsection{Review 3}
%----------- Overall evaluation -----------
SCORE: 0 (borderline paper) \newline
%----- TEXT:
Paper Overview:

This paper empirically investigates the novel Memory Bandwidth Allocation (MBA) technology, available on Intel Xeon scalable processors. The main purpose of the investigation is to 1) investigate the indirect limitation of memory bandwidth when MBA delays are applied, and 2) investigate the guaranteed memory bandwidth of a critical core (running highly critical workloads) when the MBA delays the other cores in the multi-core analysis. 

Paper Strengths:

- A novel technology (MBA) is investigated in an important context (mixed-criticality real-time system)
- Paper offers interesting observations

Paper Limitations:

- For the experiment-oriented paper (systematic evaluation as claimed by the authors), it slightly falls below the bar. The investigated workloads are not detailed enough nor justified, and there is no discussion of their limitations to the experiment setup and goals. It is not shown how the investigated delays affect the WCET values of the analyzed workloads, while this is an important aspect for real-time analysis. Also, there is no comparison to the existing approaches (MEMGUARD, etc.) that would show true benefits in real-time oriented experimentation.

- The paper is not easy to follow, there are multiple points where the paper presentation could be improved.

- The paper is motivated in the context of Virtual Machines in cloud computing environment, and safety-critical applications executing on mixed-critical real-time systems. I find it very hard to envision such a system, and the only reference for justifying this setup are the studies [8] and [9] which are more of feasibility studies than the actual motivating use cases. From my reading experience, the safety-critical applications are hardly (or even not) running on mixed-critical cloud systems.

Detailed comments:

Abstract:

It is claimed that the paper adopts a systematic measurement approach on real hardware. However, the representativeness of the investigated workloads is not discussed enough. 

Introduction:

"These safety-critical VMs must" --> Must is a strong word in this context.

"other sources of temporal contention" --> Name those.

"Memory bandwidth allocation (MBA)" --> Memory Bandwidth Allocation (MBA), also fix in the abstract

"software base-approaches" --> software-based approaches

Section II:

"(i) interference estimation" --> this is not quite the management of memory access... although it is not a huge problem.

Section III:

"exclusive LLC ... LLC exclusive" --> not the same, be sure which one is correct.

"processors, supports" --> processors, support

"we have a side effect [10]" --> What side effect? It is not enough to just reference Intel RDT

Section IV

"(tab. I)" --> Table I. Fix this appropriately for all the tables and figures. There are many such inconsistencies.

Table II is inconsistent in the categorization logic. In the first row, you have two columns (Goal) and (QUantify...) which is the description of the goal. Then, you have rows where both columns are distinctive categories. You should make the parent rows bold (e.g. Parameters and setting), and you should also make the goal as a single row single column entry. Or even it can go into the caption of the table so that it does not confuse the reader. 

"The number of observations achieves more than 99% accuracy" --> Should be described more formally. 

"a factor motivating our intuition" --> What intuition? 

"when wrtiebacks" --> when writebacks

"This explanation is plausible" --> This might be possible because...

"The second observation" --> Which is the second observation?

"from fig.2," --> Fig. 2. 

"period of 10 us" --> put microseconds

Section V:

"the latency execution" --> "the latency duration"

Section VII:

"L2 writebeacks" --> "L2 writebacks"

"mehtods" --> "methods"

As a final remark, I would suggest the authors explain in more detail the cache-related concepts such as writebacks, etc., and the investigated memory events considering Fig. 1.




\subsection{Review 4}
%----------- Overall evaluation -----------
SCORE: -2 (reject) \newline
%----- TEXT:
I am a bit irritated of your first sentence in the abstract: "Industries are recently considering the adoption of cloud computing for hosting safety critical applications." I do not believe this is true. Are you proposing that an airplane controller is now running in the cloud?

"given delay values (namely 70, 80 and 90)" what unit are you talking here?

I appreciate the exploration of Intel's MBA for real-time systems. However, I strongly think that writing/talking about safety-critical systems executing in the cloud makes no sense. Sorry, I have to reject that idea.




\section{Rebuttal}

\subsection{Response to questions (R)}
\begin{enumerate}
    \item We agree that the results might vary between different processors, however, we give a systematic method to evaluate the indirect limitation where even the L2 WB are considered as factor for a memory read workload. For this reason, we believe that this paper could be very useful for the real-time research where the memory access contention is still a well-known problem and it is suitable for this conference as supported by one of the reviewer (R2).
    \item yes, the hyperthreading can interfere in the access to the memory because the two virtual cores (on the same physical core) share the available pending requests versus the memory. The hardware (and softare) pre-fetcher can bring in cache a set of cache-lines for each LLC miss. Such behavior makes harder to achieve the maximum arrival rates in the single core analysis, furthermore, the hardware pre-fetcher is shared between the cores making difficult also the multi-core analysis.
    \item 
\end{enumerate}



\subsection{Error (E)}
\begin{enumerate}
    \item The single-core analysis consider only one core into account as we can see in Tab. II where the "core" is set to 1 as parameter. Probably, "Single-core analysis has the objective to estimate the memory access limit for an interfering core when MBA is enabled" confounded the reviewer 2, however, the interfering core represents the subject of the analysis and not a further core.
   
\end{enumerate}


\subsection{Hints (H)}
\begin{enumerate}
    \item I ritardi dell'MBA possono anche variare tra un processore e un altro, tuttavia gli esperimenti dovrebbero seguire il nostro approccio sistematico.
    \item
\end{enumerate}

\subsection{Inconsistences (I)}
\begin{enumerate}
    \item The design of experiments
    \item 
\end{enumerate}


\newpage




\begin{table}
\caption{Rebuttal}
\begin{center}
\begin{tabular}{ |c| c| c |c|}
\hline 
Observations & Reviews & Incons. & Response 
\tabularnewline
\hline 
\hline 
\textbf{+ The DOE are solid} & R1 & & 
\tabularnewline
\hline 
\textbf{+ the experiments are interesting} & R1 & &
\tabularnewline
\hline 
\textbf{+ get the difference between single and multi core analysis} & R1 & &
\tabularnewline
\hline 
\textbf{+ the topic fits in the scope of ISORC} & R2 & &
\tabularnewline
\hline 
\textbf{+ paper offer interesting observations} & R3 & &
\tabularnewline
\hline 
\textbf{+ I appreciate the exploration of Intel’s MBA for real-time 
system} & R4 & &
\tabularnewline
\hline 
- RDT is still a moving target& R1& & 1 (R)
\tabularnewline
\hline 
- the results might vary well be outdated in a few months & R1 & & 1 (R)
\tabularnewline
\hline 
- the paper should be structured more clearly and provide more details & R2 & R1 & 1 (H)
\tabularnewline
\hline 
- it is better for a workshop & R1 & R2 & 1 (R)
\tabularnewline
\hline 
- more details on CLOS and RDT & R2 & & 2 (H)
\tabularnewline
\hline 
- why Pre-fetcher and hyperthreading reduce the variability & R2 & & 2 (R)
\tabularnewline
\hline 
- Tab I and Tab II need to be explained & R2 & & 3 (H)
\tabularnewline
\hline 
- single-cores takes several cores into account (page 4) & R2 & R1 & 1 (E)
\tabularnewline
\hline 
- 99\% of accuracy & R2, R3 & & 4(H)
\tabularnewline
\hline 
- explain exclusive and inclusive architecture & R2 & & 5 (H)
\tabularnewline
\hline 
- page 4, latency cpu cycles, 64 KB? & R2 & & 3 (R)
\tabularnewline
\hline 
- MBA delay in percentage? & R2 R4 & & 5 (H)
\tabularnewline
\hline 
- How does the 2ˆ13=8192 requests relate to 512KB of memory & R2 & & 2 (E)
\tabularnewline
\hline 
- more details about the worklaods & R2, R3 & & 6 (H) 
\tabularnewline
\hline 
- interference degree example & R2 & & 3 (E)
\tabularnewline
\hline 
- no experiment setup and details & R3 & & 4 (I)
\tabularnewline
\hline 
- how the delays affect the WCET analysis & R3 & &
\tabularnewline
\hline 
- no comparison to Memguard & R3 & &
\tabularnewline
\hline 
- not easy to follow & R3 & &
\tabularnewline
\hline 
- Safety critical and RT-Cloud & R3, R4 & &
\tabularnewline
\hline 
\end{tabular}
\end{center}
\end{table}
